On the dynamical behaviour of linear higher-order cellular automata and its decidability

Higher-order cellular automata (HOCA) are a variant of cellular automata (CA) used in many applications (ranging, for instance, from the design of secret sharing schemes to data compression and image processing), and in which the global state of the system at time $t$ depends not only on the state at time $t-1$, as in the original model, but also on the states at time $t-2, \ldots, t-n$, where $n$ is the memory size of the HOCA. We provide decidable characterizations of two important dynamical properties, namely, sensitivity to the initial conditions and equicontinuity, for linear HOCA over the alphabet $\mathbb{Z}_m$. Such characterizations extend the ones shown in [23] for linear CA (LCA) over the alphabet $\mathbb{Z}^{n}_m$ in the case $n=1$. We also prove that linear HOCA of size memory $n$ over $\mathbb{Z}_m$ form a class that is indistinguishable from a specific subclass of LCA over $\mathbb{Z}_m^n$. This enables to decide injectivity and surjectivity for linear HOCA of size memory $n$ over $\mathbb{Z}_m$ using the decidable characterization provided in [2] and [19] for injectivity and surjectivity of LCA over $\mathbb{Z}^n_m$. Finally, we prove an equivalence between LCA over $\mathbb{Z}_m^n$ and an important class of non-uniform CA, another variant of CA used in many applications.

==> fps.tex <==
%======================================================
Formal power series have been successfully used in additive CA to study their dynamical 
behaviour~\cite{ManziniM99,ManziniM99a,CattaneoFMM00}. The idea is that whenever
$S$ is given a ring structure, then configurations and global rules are represented by
suitable polynomials and the application of the global rule turns into multiplications of
polynomials. Before introducing the formalism, let us fix some notation.
\begin{notation}	
For $a,b\in\N$, $\modulo{a}{b}$ means $a \mod b$. When no confusion is possible
we will adopt the same notation also for other domains than \N. For example,
$[P(X)]_b$ for a polynomial $P(X)\in\F_b[X]$ means that all coefficient are
taken mod $b$. Similarly, for a matrix $M$, the notation $[M]_b$ means that
all elements of $M$ are taken mod $b$.

Whenever $A$ is the vectorial space $\Z^n_m$, elements of $A$ and $\az$ are noted in bold. In that case, a configuration $\v\in\az$ is then a bi-infinite sequence  
$$
\v=( \dots,
\v_{-2} ,
\v_{-1} ,
\v_{0},
\v_{1} ,
\v_{2} ,
\dots )
$$
where each $\v_i$ is a vector of $\Z^n_m$.
\end{notation}

\noindent
A configuration $\v\in\CS$ can be associated with the fps
\[
P_{\v}(X)=\sum_{i\in\z}\v_i X^i
\]
\noindent
Then, if $\forall \v\in\az,\forall i\in \Z, \quad F(\v)_i = \modulo{\M_{-r}\v_{i-r}+\cdots+\M_0 \v_i+\cdots +\M_{r}\v_{i+r}}{m}$ one
finds 
\[
P_{F(\v)}(X)=\modulo{M(X) P_{\v}(X)}{m}
\]
where 
$$
M(X) =\modulo{ \sum\limits_{i=-r}^{r} \M_i X^{-i}}{m}
$$
is the finite fps associated with the MCA $F$. In this way, for any integer $t>0$ the fps associated with $F^t$ is $(M(X))^t$, and then 
$
P_{F^t(\v)}(X)=\modulo{(M(X))^t P_{\v}(X)}{m}\enspace.
$
Therefore, roughly speaking, the action of a matrix presentation over a configuration is given by multiplication in $\Z_m[X]$.

==> old-definitions.tex <==
We begin by reviewing some general notions and introducing notations we will use throughout the %rest of 
the paper.
\smallskip

\noindent
A \emph{discrete dynamical system} (DDS) is a pair $(\mathcal{X}, \mathcal{F})$ where %$(\mathcal{X}, \mathcal{d})$ 
$\mathcal{X}$ is a space equipped with a metric, \ie, a metric space, and $\mathcal{F}$ is a transformation on $\mathcal{X}$ which is continuous with respect to that metric. 
%, \ie, as pairs consisting of a metric space (with the metric defined above) and a continuous map.\\
The \emph{dynamical evolution} of a DDS $(\mathcal{X}, \mathcal{F})$  starting from the initial state $x^{(0)}\in \mathcal{X}$ is the sequence $\{x^{(t)}\}_{t\in\N}\subseteq \mathcal{X}$ where $x^{(t)}=\mathcal{F}^t(x^{(0)})$ for any $t\in\N$. 

When $\mathcal{X}=\az$ for some set finite $S$, $\mathcal{X}$ is usually equipped with the metric $d$ defined as follows
\[
\forall c,c'\in\az, \quad d(c,c')=\frac{1}{2^n}\;\quad \text{where}\;n=\min\{i\geq 0\,:\,c_i\ne
c'_i \;\text{or}\;c'_{-i}\ne c'_{-i}\}\enspace.
\]
Recall that  $\az$ is a compact, totally
disconnected and perfect topological space (\ie, $\az$ is a Cantor
space).

Any CA $\structure{S, r, f}$ defines the DDS $(\az, F)$, where $F$ is the CA global rule (which is continuous by Hedlund's Theorem~\cite{hedlund69}). From now on, for the sake of simplicity, we will sometimes identify a CA with its global rule $F$ or with the DDS $(\az, F)$. 

Recall that two DDS $(\mathcal{X},\mathcal{F})$ and $(\mathcal{X}',\mathcal{F}')$ are %\emph{isomorphic} (resp., 
\emph{topologically conjugated} if
there exists a homeomorphism $\phi: \mathcal{X} \mapsto \mathcal{X}'$ such that $\mathcal{F}'\circ \phi=\phi\circ \mathcal{F}$, while the \emph{product} of $(\mathcal{X}, \mathcal{F})$ and $(\mathcal{X}', \mathcal{F}')$ is the DDS $(\mathcal{X}\times \mathcal{X}', \mathcal{F}\times \mathcal{F}')$ where $\mathcal{F}\times \mathcal{F}'$ is defined as $\forall (x,x')\in \mathcal{X} \times \mathcal{X}'$, $(\mathcal{F}\times \mathcal{F}')(x,x')=(\mathcal{F}(x), \mathcal{F}'(x'))$ and the space $\mathcal{X}\times \mathcal{X}'$ is as usual endowed with the infinite distance. 
%$d_{\infty}$ such that $d_{\infty}(x,y)(x',y'))=\max\{d(x,x'),d(y,y')\}$ for every pair $(x,y),(x',y')\in X\times Y$.



%\renewcommand{\LP}{\ensuremath{\Z_{p^k}\left[X,X^{-1}\right]}\xspace}
\paragraph{Notations} 
For all $i,j\in\z$ with $i\leq j$ (resp., $i<j$), we write $[i,j]=\{i,i+1,\ldots,j\}$ %(resp., $[i,j)=\{i,i+1,\ldots,j-1\}$) 
to denote the interval of integers between $i$ and $j$.  For any $n\in\N$ and any set $Z$  the set of all $n\times n$ matrices with coefficients in $Z$ and the set of Laurent polynomials with coefficients in $Z$ will be noted by $\mat{n}{Z}$ and $\LP$, respectively. In the sequel, bold symbols are used to denote vectors, matrices, and configurations over a set of states which is a vectorial space. Moreover, 
$m$ will be an integer bigger than $1$ and $\Z_m=\{0, 1, \ldots, m-1\}$  the ring with the usual sum and product modulo $m$. For any $\x\in\Z^n$ (resp., any matrix $\M(X)\in\mat{n}{\LPZ}$), we will denote by $\modulo{\x}{m}\in\Z_m^n$ (resp., $\modulo{\M(X)}{m}$),  the vector (resp., the matrix) in which each component $x^i$ of $\x$ (resp., every coefficient of each element of $\M(X)$) is taken modulo $m$. Finally, for any matrix $\M(X)\in\LPm$ and any $t\in\N$, the $t$-th power of $\M(X)$ will be noted more simply by $\M^t(X)$ instead of $(\M(X))^t$.
%%
\begin{definition}[HOCA]
\begin{comment}
A \emph{$k$-th order CA (HOCA)} is a structure
$\mathcal{H}=\structure{k,S,r,h}$ where $k\in\N$ is the \emph{memory} size, $S$ is the \emph{alphabet}, $r\in\N$ is the \emph{radius}, and $f\colon S^{(2r+1)k}\to S$ is the \emph{local rule}. The \emph{dynamical evolution} of an HOCA $\mathcal{H}$  starting from the initial configurations $c^{(0)},c^{(1)},\ldots,c^{(k-1)}\in\az$ is the sequence $\{c^{(t)}\}_{t\in\N}\subset \az$ defined for any $t\geq k$ as follows 
%
%\emph{global rule} $H:\az\to\az$ defined as
\[
\quad \forall i\in\Z,\quad  c_i^{(t)}=h\left(\quad \begin{matrix} c^{(t-k)}_{[i-r, i+r]}\\ \\ c^{(t-k+1)}_{[i-r, i+r]}\\ \vdots\\ \\c^{(t-1)}_{[i-r, i+r]}\end{matrix}\quad \right)
\]
OPPURE (SE SI SCRIVONO LE PROPRIETA' DINAMICHE PER GLI HOCA)
\\
\end{comment}
A \emph{$k$-th order CA (HOCA)} is a structure
$\mathcal{H}=\structure{k,S,r,h}$ where $k\in\N$ is the \emph{memory} size, $S$ is the \emph{alphabet}, $r\in\N$ is the \emph{radius}, and $h\colon S^{(2r+1)k}\to S$ is the \emph{local rule}. Any HOCA $\mathcal{H}$ induces the \emph{global rule} $H:\left({\az}\right)^k\to\left({\az}\right)^k$ associating any vector $\myvec{e}=(e^1, \ldots, e^k)\in \left({\az}\right)^k$ of $k$ configurations of $\az$ with the vector $H(\myvec{e})\in\left({\az}\right)^k$ such that $H(\myvec{e})^j=e^{j+1}$ for each $j\neq k$ and
\[
\quad \forall i\in\Z,\quad H(\myvec{e})^k_i=h\left(\begin{matrix} e^{1}_{[i-r, i+r]}\\ \\ e^{2}_{[i-r, i+r]}\\ \vdots\\ e^{k}_{[i-r, i+r]}\end{matrix}\right)
\]
In this way, $\mathcal{H}$ defines the DDS $\left(\left({\az}\right)^k, H\right )$. As with CA we identify a HOCA with its global rule or the DDS defined by it. 
\begin{comment}
 the \emph{dynamical evolution} of %an HOCA 
$\mathcal{H}$  starting from the initial configuration vector $\ccc^{(0)}\in \left({\az}\right)^k $%=(c^{(0)},c^{(1)},\ldots,c^{(k-1)})\in \left({\az}\right)^k$ 
is the sequence $\{\ccc^{(t)}\}_{t\in\N}\subset \left({\az}\right)^k$ where $\ccc^{(t)}=H^t(\ccc^{(0)})$ for any $t\in\N$.
\end{comment}
\end{definition}
%%
\begin{remark}
It is easy to check that for any HOCA $\mathcal{H}=\structure{k,S,r,h}$ there exists a CA $\structure{S^k,r,f}$ which is topologically conjugated to $\mathcal{H}$.
\end{remark}

The study of the dynamical behaviour of HOCA is still at its early stages; a few results are known for the class of \emph{linear HOCA}, namely, those HOCA defined by a local rule $f$  which is \emph{linear}, \ie,  $S$ is %the ring 
$\Z_m$ %=\{0, 1, \ldots, m-1\}$
%  with the usual sum and product modulo $m$, 
and there exist coefficients $a^j_i\in\Z_m$  ($j=1, \ldots, k$ and $i=-r, \ldots, r$) such that for any element
\[
\x=\left(\begin{matrix} x^{1}_{-r} & \hdots &  x^{1}_{r} \\ \\ x^{2}_{-r} & \hdots &  x^{2}_{r}\\ \vdots\\ x^{k}_{-r} & \hdots &  x^{k}_{r}\end{matrix}\right)\in \Z_m^{(2r+1)k}, \quad f(\x)=\modulo{\sum_{j=1}^{k}\sum_{i=-r}^{r} a^j_i x^{j}_{i}}{m}\enspace .
\]  
%where $\modulo{x}{m}$ is the integer $x$ taken modulo $m$. 
It is easy to see that linear HOCA are additive, \ie, 
\[
\forall\myvec{c},\myvec{d}\in \left(\Z_m^{\Z}\right)^k, \quad  H(\myvec{c}+\myvec{d})=
H(\myvec{c})+H(\myvec{d})
\]
where, with the usual abuse of notation, $+$ denotes the natural extension of the sum over $\Z_m$ to both $\Z_m^{\Z}$ and $\left(\Z_m^{\Z}\right)^k$.

In~\cite{bruyn1991}, a much more convenient representation is introduced for the case of linear HOCA (in dimension $d=1$) by means of the following notion.
%\noindent\paragraph{Standing assumption} $S$ is assumed to be the additive
%group $\Z_m$ for $m\in\N$, the global rule is additive and the dimension $d$ is $1$.
%From now on, we share the same assumptions.


\begin{definition}[Linear Cellular Automata]
A \emph{Linear Cellular Automaton} (LCA) is a CA $\mathcal{L}=\structure{\Z_m^n, r, f}$ where the local rule $f\colon(\Z_m^n)^{2r+1}\to\Z_m^n$ is defined by $2r+1$ matrixes  
$\M_{-r},\ldots, \M_0,\ldots, \M_r\in\mat{n}{\Z_m}$ 
%$A_{-r},\ldots, A_0,\ldots, A_r\in\mat{n}{\Z_m}$ 
as follows: 
$f(\x_{-r}, \ldots,\x_0,\ldots,\x_r) = 
\modulo{\sum_{i=-r}^r \M_i\cdot\x_i}{m}$ for any 
$(\x_{-r}, \ldots,\x_0,\ldots,\x_r)\in(\Z_m^n)^{2r+1}$.
\end{definition}
\begin{remark}
LCA have been strongly investigated in the case $n=1$ and all the dynamical properties have been characterized in terms of the $1\times 1$ matrices (\ie, coefficients) defining the local rule, in any dimension too~\cite{ManziniM99, CattaneoDM04}.  
\end{remark}



We recall that any linear HOCA $\mathcal{H}$ can be simulated by a suitable LCA, as shown in~\cite{bruyn1991}. Precisely, given a linear HOCA $\mathcal{H}=\structure{k,\Z_m,r,h}$, where $h$ is defined by the coefficients $a^j_i\in\Z_m$, the LCA simulating $\mathcal{H}$ is $\mathcal{L}=\structure{\Z_m^k, r, f}$  with $f$ defined by following matrices 
%\[
\begin{align}
\label{M0}
\M_0=
\begin{bmatrix}
0&1&0& \dots&0&0\\
0&0& 1&\ddots&0&0\\
0&0&0 &\ddots&0&0\\
\vdots&\vdots& \vdots&\ddots&\ddots&\vdots\\
%0&0&0&0&1&0&0\\
%0&0&0&0&0&1&0\\
0        &   0 &0   & \dots &0&1\\
a_0^1&a_0^2& a_0^3 &\dots &a_0^{k-1}&a_0^k
\end{bmatrix}\enspace,
%\]
\end{align}
and, for $i\in [-r, r]$ with $i\ne0$,
%\[
\begin{align}
\label{Mi}
\M_i=
\begin{bmatrix}
0&0&0&\dots&0&0\\
0&0&0&\dots&0&0\\
0&0&0&\dots&0&0\\
\vdots&\vdots&\vdots& \ddots&\vdots&\vdots\\
%0&0&0&0&1&0&0\\
%0&0&0&0&0&1&0\\
0        &   0    & 0 &  \dots &0&0\\
a_i^1&a_i^2& a_i^3& \dots &a_i^{k-1}&a_i^k
\end{bmatrix}\enspace.
\end{align}
%\]
\begin{remark}
\label{rem:classes}
We want to put in evidence that a stronger result actually holds (easy proof, important remark): any linear HOCA $\mathcal{H}$ is topologically conjugated to the LCA $\mathcal{L}$ defined by the matrices in~\eqref{M0} and~\eqref{Mi}. %$\M_{-r},\ldots, \M_0,\ldots, \M_r$ above introduced. 
Clearly, the converse also holds: for any LCA %$\mathcal{L}$  
defined by the matrices in~\eqref{M0} and~\eqref{Mi} %$\M_{-r},\ldots, \M_0,\ldots, \M_r$ 
there exists a linear HOCA which is topologically conjugated to it. In other words, up to a homeomorphism the whole class of linear HOCA is identical to the subclass of LCA defined by the matrices above introduced.
% $\structure{\Z_m^n, r, f}$, 
In the sequel, we will call $\mathcal{L}$ the \emph{matrix presentation} of $\mathcal{H}$.  
%, which is  defined %by the matrixes $\M_{-r},\ldots, \M_0,\ldots, \M_r$ above introduced. 
\end{remark}

We are now going to show a stronger and useful new fact, namely, that the class of linear HOCA is nothing but the subclass of LCA represented by a formal power series which is a matrix in Frobenius normal form. Before proceeding, let us recall the  \emph{formal power series} (fps)
%
\begin{comment}
%%%TUTTA ROBA DI ENRICO
\begin{definition}[Matrix presentation]
Given an additive \HOCA\ $\mathcal{A}\equiv\structure{1,\Z_m,\set{-r,\ldots,0,\ldots,r},k,\delta}$, define a set of square matrices $M_{-r},\ldots,M_0,\ldots,M_r$ such that
\[
M_0=
\begin{bmatrix}
0&1&0&0&\dots&0&0\\
0&0&1&0&\dots&0&0\\
\vdots&&\ddots&\ddots&\ddots&\vdots&\vdots\\
0&0&0&0&1&0&0\\
0&0&0&0&0&1&0\\
0&0&0&0&\dots&0&1\\
0&0&0&0&\dots&0&\lambda_0
\end{bmatrix}
\]
and for $i\ne0$
\[
M_i=
\begin{bmatrix}
0&0&0&0&\dots&0&0\\
0&0&0&0&\dots&0&0\\
\vdots&&\ddots&\ddots&\ddots&\vdots&\vdots\\
0&0&0&0&0&0&0\\
0&0&0&0&0&0&0\\
0&0&0&0&\dots&0&0\\
0&0&0&0&\dots&0&\lambda_i
\end{bmatrix}
\]
for suitable $\lambda_0,\lambda_i\in\Z_m$.
The \emph{matrix presentation} of $\mathcal{A}$ is
the structure $\structure{r,M_{-r},\ldots,M_0,\ldots,M_r,\delta'}$ where
is the \emph{radius}, $M_i\in\mat{k+1}{\Z_m}$ (for $i\in[-r,r]$) are the \emph{local matrices} 
and $\delta'\colon(\Z_m^{k+1})^{2r+1}\to\Z_m$ is the \emph{local rule} such that
$\delta'(\v_{-r}, \ldots,\v_0,\ldots,\v_r) = \sum_{i=-r}^r M_i\cdot\v_i$ for all
$(\v_{-r}, \ldots,\v_0,\ldots,\v_r)\in(\Z_m^{k+1})^{2r+1}$.
\end{definition}

The matrices of the previous definition are very peculiar. However, one may
think to adopt more general matrices which does not necessarily correspond
to an additive \HOCA. Indeed, consider the following example.

\begin{example}
Consider the following matrix presentation of an \HOCA\ of state set $\Z_2$, radius $1$ and
\[
M_{-1}=
M_0=
\begin{bmatrix}
0&0\\
0&0
\end{bmatrix}
\qquad
M_1=
\begin{bmatrix}
1&0\\
0&1
\end{bmatrix}
\]
This is the \emph{left shift} map since the initial configuration is shifted left
of one position at every step. Indeed, consider the following
configuration
\[
\myvec{v}\equiv\left(\ldots\binom{a}{b}_{-1}\binom{c}{d}_0\binom{e}{f}_1\ldots\right)
\]
We have $M_{-1}\cdot(a\ b)+M_0\cdot(c\ d)+M_1\cdot(e\ f)=\binom{0}{0}+\binom{0}{0}
+\binom{e}{f}$ and hence
\[
F_\delta(\myvec{v})\equiv\left(\ldots\binom{e}{f}_0\ldots\right)
\]
\end{example}
\end{comment}
\noindent
%
which have been successfully used to study the dynamical 
behaviour of LCA in the case $n=1$~\cite{ito83,ManziniM99,ManziniM99a,CattaneoFMM00}. The idea of this formalism is that configurations and global rules are represented by
suitable polynomials and the application of the global rule turns into multiplications of
polynomials. 
In the more general case of LCA over $\Z_m^n$,  a configuration $\ccc\in(\Z_m^n)^\Z$ can be associated with the fps
\[
\P_{\ccc}(X)=\sum_{i\in\z}\ccc_i X^i = 
\begin{bmatrix}
c^1(X)\\
\vdots\\
c^n(X)
\end{bmatrix}
=
\begin{bmatrix}
\sum_{i\in\Z} c_i^1 X^i\\
\vdots\\
\sum_{i\in\Z} c_i^n X^i
\end{bmatrix}\in\left(\LPm\right)^n\cong \LPmn \enspace.
\]
\noindent
Then, if 
%$\forall \v\in\az,\forall i\in \Z, \quad F(\v)_i = \modulo{\M_{-r}\v_{i-r}+\cdots+\M_0 \v_i+\cdots +\M_{r}\v_{i+r}}{m}$ 
$F$ is the global rule of a LCA defined by $\M_{-r},\ldots, \M_0,\ldots, \M_r$, one finds 
\[
\P_{F(\ccc)}(X)=\modulo{\M(X) \P_{\ccc}(X)}{m}
\]
where 
$$
\M(X) =\modulo{ \sum\limits_{i=-r}^{r} \M_i X^{-i}}{m}
$$
is the finite fps associated with the LCA $F$. In this way, for any integer $t>0$ the fps associated with $F^t$ is $\M(X)^t$, and then 
$
\P_{F^t(\ccc)}(X)=\modulo{\M(X)^t \P_{\ccc}(X)}{m}\enspace.
$ 
Roughly speaking, the action of a LCA over a configuration is given by multiplication between elements of $\mat{n}{\LPm}$ with elements of $\left(\LPm\right)^n$. Throughout this paper, $\M(X)^t$ will refer to $\modulo{\M(X)^t}{m}$. 
%\textbf{Therefore, roughly speaking, the action of a matrix presentation over a configuration is given by multiplication in $\Z_m[X]$}.

%Denote $\LP$ the set of Laurent polynomials with coefficients over $\Z_{m}$. 
%We are interested in the degrees of such polynomials both \wrt $X$ and $X^{-1}$.
 

A matrix $\M(X)\in\mat{n}{\LP}$ is in \emph{Frobenius normal form} if  
\begin{eqnarray}
\label{FNF}
\M(X)=
\begin{comment}
\begin{bmatrix}
0&1&0& \dots&0&0\\
0&0& 1&\ddots&0&0\\
0&0&0 &\ddots&0&0\\
\vdots&\vdots& \vdots&\ddots&\ddots&\vdots\\
%0&0&0&0&1&0&0\\
%0&0&0&0&0&1&0\\
0        &   0 &0   & \dots &0&1\\
\pp_1(X)&\pp_2(X)& \pp_3(X) &\dots &\pp_{n-1}(X)&\pp_{n}(X)
\end{bmatrix}\\
\end{comment}
\begin{bmatrix}
0&1&0& \dots&0&0\\
0&0& 1&\ddots&0&0\\
0&0&0 &\ddots&0&0\\
\vdots&\vdots& \vdots&\ddots&\ddots&\vdots\\
\\
%0&0&0&0&1&0&0\\
%0&0&0&0&0&1&0\\
0        &   0 &0   & \dots &0&1\\
%\medskip
\\
\mm_0(X)&\mm_1(X)& \mm_2(X) &\dots &\mm_{n-2}(X)&\mm_{n-1}(X)
\end{bmatrix}
\end{eqnarray}
\begin{comment}
\[
M(X)=
\begin{bmatrix}
0&1&0& \dots&0&0\\
0&0& 1&\ddots&0&0\\
0&0&0 &\ddots&0&0\\
\vdots&\vdots& \vdots&\ddots&\ddots&\vdots\\
%0&0&0&0&1&0&0\\
%0&0&0&0&0&1&0\\
0        &   0 &0   & \dots &0&1\\
c_0(X)&c_1(X)& c_2(X) &\dots &c_{n-2}(X)&c_{n-1}(X)
\end{bmatrix}
\]
\end{comment}
\begin{comment}
\[
M(X) =\begin{bmatrix}
 0& \cdots & \cdots   &  0 &   | \\
1  & \ddots &  &\vdots  &  |\\
0  &\ddots  &\ddots  &\vdots  & \myvec{c}(X) \\
\vdots   &  & \ddots & 0 &  |\\
 0   & \cdots & 0 & 1 &  | \\
 \end{bmatrix} 
\]
\end{comment}
%for some vector 
%$\myvec{c}(X)=\begin{bmatrix} c_0(X)\\ c_1(X)\\ \vdots\\ c_{n-1}(X)\end{bmatrix}$
%%% PRECEDENTEwhere each $\pp_i(X)\in\LP$. %ciao $\pp^M(X)$
where each $\mm_i(X)\in\LP$

From now on, for a  given matrix $\M(X)\in\mat{n}{\LP}$ in Frobenius normal form, $\myvec{\mm}(X)$ 
%$\myvec{\pp}(X)$
will always make reference to its $n$-th row. %column vector. 



\begin{definition}{\blue (Frobenius LCA)}\label{frobeniusLCA}
%Let $p$ be a prime number and $k\geq 1$. 
A LCA $F$ over the alphabet $\Z^n_{m}$ is said to be a \emph{Frobenius LCA} if the fps $\M(X)\in\mat{n}{\LPm}$ associated with $F$ is in Frobenius normal form. 
\end{definition}
\begin{comment}
$$
\begin{bmatrix}
 0& \cdots & \cdots   &  0 &c_0(X)    \\
1  & \ddots &  &\vdots  &c_1(X)  \\
0  &\ddots  &\ddots  &\vdots  &\vdots  \\
\vdots   &  & \ddots & 0 & \vdots \\
 0   & \cdots & 0 & 1 & c_{n-1}(X)  \\
 \end{bmatrix} 
$$
where each $c_i(X)$ is a Laurent polynomial with coefficients belonging to $\Z_{p^k}$.
\end{comment}
\begin{comment}
Sia $F$ un MCA di frobenius definito come segue.
$$F =\begin{bmatrix}
 0& \cdots & \cdots   &  0 &c_0    \\
1  & \ddots &  &\vdots  &c_1  \\
0  &\ddots  &\ddots  &\vdots  &\vdots  \\
\vdots   &  & \ddots & 0 & \vdots \\
 0   & \cdots & 0 & 1 & c_{n-1}  \\
 \end{bmatrix} 
$$
con $c_i$ polinomi di Laurent con coefficienti in $\Z_{p^k}$ con $k\geq 1$ e $p$ primo.
\end{comment}
%%
%\begin{remark}
\begin{comment}
Since for any given configuration $\ccc\in (\Z_m^n)^{\Z}$
\[
P_{\ccc}(X) = 
\begin{bmatrix}
c^1(X)\\
\vdots\\
c^n(X)
\end{bmatrix}
=
\begin{bmatrix}
\sum_{i\in\Z} c_i^1 X^i\\
\vdots\\
\sum_{i\in\Z} c_i^n X^i
\end{bmatrix}
\]
\end{comment}
\begin{comment}
Remark that the action of a Frobenius LCA $F$ over any given configuration $\ccc\in (\Z_m^n)^{\Z}$ is such that
\[
\P_{F(\ccc)}(X) = \M(X) \P_{\ccc}(X) =
\begin{bmatrix}
c^2(X)\\
\vdots\\
\sum_{i=1}^n \pp_i(X) c^i(X)
\end{bmatrix} \enspace.
\]
\end{comment}
%PARLARE DI CONIUGAZIONE TOPOLOGICA
%This allows us to state the following
It is immediate to see that a LCA is a Frobenius one iff it is defined by the matrices in~\eqref{M0} and~\eqref{Mi}, \ie, iff it is topologically conjugated to a linear HOCA. This fact together with Remark~\ref{rem:classes} and Definition~\ref{frobeniusLCA}, allow us to state the following
%
\begin{proposition} Up to a homeomorphism, the class of linear HOCA is nothing but the class of Frobenius LCA.
\end{proposition}

At this point we want to stress that the action of a Frobenius LCA $F$, or, equivalently, a linear HOCA, over a configuration $\ccc\in (\Z_m^n)^{\Z}$ can be viewed as a bi-infinite array of \emph{linear--feedback shift register}. %~\cite{}. 
Indeed, it holds that
\[
\P_{F(\ccc)}(X) = \M(X) \P_{\ccc}(X) =
\begin{bmatrix}
c^2(X)\\
\vdots\\
\sum_{i=1}^n \mm_{i-1}(X) c^i(X)
\end{bmatrix} \enspace,
\]
where the $n$--th component of the vector $\P_{F(\ccc)}(X)$ is given by the sum of the results of the actions of $n$ one-dimensional LCA over $\Z_m$ each of them applied on a different component of $\P_{\ccc}(X)$, or, in other words, on a different element of the memory of the linear HOCA which is topologically conjugated to $F$.

\begin{comment}
As a consequence, given a Frobenius LCA $F$, for any configuration \ccc\in (\Z_m^n)^{\Z}$

 the $n$th component of the vector $\P_{F(\ccc)}(X)$ is given by the sum of the results of the actions of $n$ one-dimensional LCA over $\Z_m$ each of them applied on a different component of $\P_{\ccc}(X)$, or, in other words, on a different element of the memory of the linear HOCA.

HOCA LINEAR SHIFT REGISTER
\end{comment}
%of a Frobenius LCA $F$ over any given configuration $\ccc\in (\Z_m^n)^{\Z}$is given by the sum of $n$ one-dimensional LCA over $\Z_m$ each of them applied on one element of the history / memory HOCA LINEAR SHIFT REGISTER
%\end{remark}
\begin{comment}
\begin{proposition} Gli HOCA sono esattamente gli MCA la cui fps e' una matrice di Frobenius.
\end{proposition}
\end{comment}
\begin{remark}
Actually, in literature a matrix is in Frobenius normal form if either it or its transpose has a form as in~\eqref{FNF}. Since any matrix in Frobenius normal form is conjugated to its transpose, any Frobenius LCA $F$ is topologically conjugated to a LCA $G$ such that the fps associated with $G$ is the transpose of the fps associated with $G$. In other words, up to a homeomorphism, such LCA $G$, linear HOCA, and Frobenius LCA form the same class and, in particular, the action of $G$ on any configuration $\ccc\in (\Z_m^n)^{\Z}$ is such that
\begin{comment}%%PRECEDENTE
\[
\P_{G(\ccc)}(X) = \M(X)^T \P_{\ccc}(X) =
\begin{bmatrix}
\pp_1(X) c^n(X)\\
c^1(X) + \pp_2(X)c^n(X) \\
\vdots\\
c^{n-1}(X) + \pp_n(X)c^n(X)
\end{bmatrix} \enspace,
\]
\end{comment}
\[
\P_{G(\ccc)}(X) = \M(X)^T \P_{\ccc}(X) =
\begin{bmatrix}
\mm_0(X) c^n(X)\\
c^1(X) + \mm_1(X)c^n(X) \\
\vdots\\
c^{n-1}(X) + \mm_{n-1}(X)c^n(X)
\end{bmatrix} \enspace,
\]
where $\M(X)^T$ is the transpose of the matrix $\M(X)$ associated to the LCA $F$ which is topologically conjugated to $G$.
%LCA $F$ that is a  Frobenius LCA according to ... is topologically conjugated to a LCA $G$ such that the fps associated with  $G$ is the transpose of the fps associated to $F$
%
%formal both a matrix and its transpose are considered matrices in Frobenius normal form. Dire rapidamente che le matrici di frobenius sono anche quelle la cui trasposta e' quella definita come sopra. 
%
%Gli MCA di Frobenius colonna sono top coniugati con quelli riga. Per cui la classe dei Frobenius colonna coincide con la classe dei frobenius riga che coincide con gli HOCA. I Frobenius colonna, analizzati per i fatti loro visti agiscono cosi: FORMULA.
\end{remark}
%
From now on, we will focus on Frobenius LCA, \ie, matrix presentations of linear HOCA.  Indeed, they allow convenient algebraic manipulations that are very useful to study formal properties of linear HOCA. For example, in~\cite{bruyn1991} and~\cite{kari2000}, the authors proved decidable characterization for injectivity and surjectivity for LCA in terms of the matrix $\M(X)$ associated to them. We want to stress that, by Remark~\ref{rem:classes} and Definition~\ref{frobeniusLCA}, one can use these characterizations for deciding injectivity and surjectivity of linear HOCA.

In this paper we are going to adopt a similar attitude, \ie, we are going to characterise
the dynamical behaviour of linear HOCA by the properties of the matrices in their matrix
presentation. %$\mathscr{P}$ 
\begin{comment}From now on, we will focus on matrix presentations and turn back to \HOCA\ only
when the general results have to be specialised to \HOCA\ case. 
Indeed, the matrix representation allows convenient algebraic manipulations.
For example, in~\cite{bruyn1991}, the authors proved that a \HOCA\ 
is reversible if and only if some matrix built from the local rule is invertible.
%%% c-era a cap[o
In this paper we are going to adopt a similar attitude, we are going to characterize
the dynamical behaviour of \HOCA\ by the properties of the matrices in their matrix
presentation. The next section provides further motivations for the study of \HOCA\
and the following one will introduce all the basic notions to precisely state
the new results.
\end{comment}


==> old-dyn.tex <==
In this paper we are particularly interested to the so-called \emph{sensitivity to the initial conditions} and \emph{equicontinuity}. As dynamical properties, they represent the main features of instable and stable DDS, respectively. The former is the well-known basic component and essence of the chaotic behavior of DDS, while the latter is a strong form of stability.

Let $(\mathcal{X}, \mathcal{F})$ be a DDS. 
The DDS $(\mathcal{X}, \mathcal{F})$ is \emph{sensitive to the initial conditions} (or simply \emph{sensitive}) if there exists $\varepsilon>0$ such that for any $x\in \mathcal{X}$ and any
$\delta>0$ there is an element $y\in \mathcal{X}$ such that
$d(y,x)<\delta$ and $d(\mathcal{F}^n(y),\mathcal{F}^n(x))>\varepsilon$
for some $n\in\n$. Recall that, by Knudsen's Lemma~\cite{knudsen94}, $(\mathcal{X}, \mathcal{F})$ is sensitive iff $(\mathcal{Y}, \mathcal{F})$ is sensitive where $\mathcal{Y}$ is any dense subset of $\mathcal{X}$ which is $\mathcal{F}$-invariant, \ie,  $\mathcal{F}(\mathcal{Y})\subseteq\mathcal{Y}$.%In~\cite{Ku97}, K\r{u}rka 
%proved that the following conditions are equivalent: $F$ is not sensitive; $F$ is almost equicontinuous;  $F$ admits a $r$-blocking word.\\

In the sequel, we will see that in the context of LCA an alternative way to study sensitivity is via equicontinuity points. An element $x\in \mathcal{X}$ is an \emph{equicontinuity point} for $(\mathcal{X}, \mathcal{F})$ if $\forall\varepsilon>0$
there exists $\delta>0$ such that for all $y\in \mathcal{X}$, $d(x,y)<\delta$ implies that $d(\mathcal{F}^n(y),\mathcal{F}^n(x))<\varepsilon$ for all $n\in\n$. The system $(\mathcal{X}, \mathcal{F})$ is said to be \emph{equicontinuous} if $\forall\varepsilon>0$ there exists $\delta>0$ such that for all $x,y\in \mathcal{X}$,
$d(x,y)<\delta$ implies that $\forall n\in\n,\;d(\mathcal{F}^n(x),\mathcal{F}^n(y))<\varepsilon$.  
%, while
%it is said to be \emph{almost equicontinuous} if the set $E$ of its equicontinuity points is residual (\ie, $E$ contains a countable intersection of dense open subsets). 
Recall that any CA $(\az, F)$ is equicontinuous if and only if there exist two integers $q\in\n$ and  $p>0$ such that $F^q=F^{q+p}$~\cite{Ku97}. Moreover, for the subclass of LCA defined by $n=1$ the following result holds:
\begin{theorem}[\cite{ManziniM99}]
Let %$\mathcal{L}=\structure{\Z_m, r, f}$ 
$(\Z_m^{\Z}, F)$ be a LCA where the local rule $f\colon(\Z_m)^{2r+1}\to\Z_m$ is defined by $2r+1$ coeffiecients  
$m_{-r},\ldots, m_0,\ldots, m_r\in\Z_m$. Denote by $\mathcal{P}$ the set of prime factors of $m$. The following statements are equivalent:
\begin{enumerate}
\item $F$ is sensitive to the initial conditions;
\item $F$ is not equicontinuous;
\item  there exists a prime number $p\in\mathcal{P}$ which does not divide $\gcd(m_{-r},\ldots, m_{-1},m_{1},\ldots, m_r)$.
\end{enumerate}
\end{theorem}  
The dichotomy between sensitivity and equicontinuity still holds for general LCA.
\begin{proposition}\label{prop:dich}
Let $\mathcal{L}=\structure{\Z_m^n, r, f}$ be a LCA where the local rule $f\colon(\Z_m^n)^{2r+1}\to\Z_m^n$ is defined by $2r+1$ matrices  
$\M_{-r},\ldots, \M_0,\ldots, \M_r\in\mat{n}{\Z_m}$. The following statements are equivalent:
\begin{enumerate}
\item $F$ is sensitive to the initial conditions;
\item $F$ is not equicontinuous;
%\item \lim\sup_{t\to\infty} .
\item $\left | \{\M(X)^i, i\geq 1 \} \right | = \infty$.
\end{enumerate}
\end{proposition}
\begin{proof}
The equivalence between $1.$ and $2.$ is a consequence of linearity of $F$ and the Knudsen's Lemma applied on the subset of the finite configurations, \ie, those having a state different from the null vector only in a finite number of cells. Finally, if condition $3.$ is false, then $F$ is equicontinuous, that is $2.$ is false too.
\qed
\end{proof}
An immediate  consequence of Proposition~\ref{prop:dich} is that any characterization of sensitivity to the initial conditions in terms of the matrices defining LCA over $\Z_m^n$ would also provide a characterization of equicontinuity. In the sequel, we are going to show that such a characterization actually exists. First of all, we recall a result that helped in the investigation of dynamical properties in the case $n=1$ and we now state it in a more general form %to be useful 
for LCA over $\Z_m^n$ (immediate generalisation of the result in~\cite{}). 

Let $\left ( (\Z_m^n)^{\Z}, F \right)$ be a LCA and let $q$ be any factor of $m$. 
%For any configuration $\ccc\in (\Z_m^n)^{\Z}$, we will denote by $\modulo{\ccc}{q}$  the configuration in $(\Z_q^n)^{\Z}$ defined as 
We will denote by $\modulo{F}{q}$ the map $\modulo{F}{q}: (\Z_q^n)^{\Z}\to (\Z_q^n)^{\Z}$ defined as $\modulo{F}{q}(\ccc)=\modulo{F(\ccc)}{q}$, for any $\ccc\in(\Z_q^n)^{\Z}$.
\begin{lemma}[\cite{CattaneoDM04, DamicoMM03}]
\label{lem:dec}
Consider any LCA  $\left ( (\Z_m^n)^{\Z}, F \right)$  with $m=pq$ and $\gcd(p,q)=1$. It holds that the given LCA is topologically conjugated to $\left ( (\Z_p^n)^{\Z} \times (\Z_q^n)^{\Z}, \modulo{F}{p}\times\modulo{F}{q} \right)$.
\end{lemma}
\begin{comment}
\begin{proof}

\end{proof}
\end{comment}
As a consequence of Lemma~\ref{lem:dec}, if $m=p_1^{k_1} \cdots p_l^{k_l}$ is the prime factor decomposition of $m$, any LCA over $\Z_m^n$  is topologically conjugated to the product of LCAs over $\Z^n_{p_{i}^{k_i}}$. %So all the properties which are preserved under product and under topological conjugacy are lifted from LCA over $\Z_{p^{k} }^n$ to LCA over $\Z_{m}^n$. Since sensitivity and equicontinuity are among these properties,
Since sensitivity is preserved under topological conjugacy for DDS over a compact space and the product of two DDS is sensitive if and only if at least one of them is sensitive, we will study sensitivity for Frobenius LCA over $\Z_{p^{k}}^n$. We will show a decidable characterization of sensitivity to the initial conditions for Frobenius LCA over $\Z_{p^{k}}^n$ (Lemma~\ref{frobeniusSensitivity}). Such a decidable characterization together with the previous remarks about the decomposition of $m$, the topological conjugacy involving  any LCA over $\Z_m^n$  and the product of LCAs over $\Z^n_{p_{i}^{k_i}}$, and how sensitivity behaves with respect to a topological conjugacy and the product of DDS, immediately lead to state the main result of the paper.
\begin{theorem}\label{main}
Sensitivity and Equicontinuity are decidable for Frobenius LCA over $\Z_m^n$, or, equivalently, for HOCA over $\Z_m$.
\end{theorem}

 %we will study them for Frobenius LCA over $\Z_{p^{k} }^n$. 
%If $F$ is both equicontinuous and surjective then there exists an integer $p>0$ such that $F^p(x)=x$ for all configurations $x\in\az$.\\
%
%Equicontinuity/sensitivity are strong features of stability/instability for a DDS.  Furthermore, sensitivity represents the essence of the chaotic behavior of DDS.I

%In this paper we are interested to \emph{sensitivity to initial conditions}. 
%This a well-known basic component of many chaotic behaviors. 
%A \HOCA\ of global rule $F_\delta$ is sensitive to initial conditions if and only if
%there exists some $\varepsilon>0$ such that for all configurations $x\in\CS$
%and for all $\xi>0$ there exists $y\in\mathcal{B}_\xi(x)$ and $t\in\N$ such that
%$d(F_\delta^t(x),F_\delta^t(y))>\varepsilon$.
\begin{comment}
 Recall that a configuration $x\in\CS$ is an
\emph{equicontinuity point} for a \HOCA\ of global rule $F_\delta$ iff for all
$\varepsilon>0$ there exists $\xi>0$ such that for all $y\in\mathcal{B}_\xi(x)$
it holds $d(F_\delta^t(x),F_\delta^t(y))<\varepsilon$. Denote $E(F_\delta)$ the set of all
equicontinuity points of the \HOCA\ $F_\delta$. An \HOCA\ is \emph{equicontinuous}
iff $E(F_\delta)=\CS$. Remark that by the additivity property,
additive \HOCA\ are such that $E(F_\delta)=\emptyset$ or $E(F_\delta)=\CS$.

In other words, \HOCA s are either sensitive or equicontinuous.
Therefore, in the case of additive \HOCA, characterizing sensitivity to initial conditions
is the same as characterizing equicontinuity.
\\
\end{comment}
%======================================================
%======================================================
\begin{comment}
Sia $X$ una configurazione, $F$ un MCA, $m=p q$, $p$ e $q$ coprimi, $n\geq 1$.
%\begin{comment}
$$\begin{tikzcd}
  \modulo{X}{m} \arrow[r, " \modulo{F^n}{m}"] \arrow[d,"\modulo{\cdot}{p}\ \modulo{\cdot}{q}"]                                             &        \modulo{X}{m}\arrow[d,"\modulo{\cdot}{p}\ \modulo{\cdot}{q}"] \\
  \modulo{X}{p},\modulo{X}{q} \arrow[r, "\ \ \ \modulo{F^n}{p}\ \modulo{F^n}{q}\ \ \ "]    &       \modulo{X}{p},\modulo{X}{q}\end{tikzcd}
$$
%\end{comment}
\end{comment}



==> old-frobe.tex <==
%======================================================
\section{Sensitivity of Frobenius LCA over $\Z^n_{p^k}$}
%======================================================
%======================================================
%Let $\LP$ be the set of the Laurent polynomials with coefficients belonging to a ??? ring???.
% Let $\LPK$ be the set of Laurent polynomials with coefficients belonging to $\Z_{p^k}$.
% MI SEMBRA CHE L'INSIEME PIU' GROSSO $\LP$ SERVA SOLO PER DIMOSTRARE (vedi Teorema molto piu' avanti) LA RICORRENZA  T(m)= un polinomio x T(m-1)+ un polinomio x T(m-2)... ecc CHE NON VALE SOLO SE I COEFFICIENTI SONO SU ZPK
 
%\renewcommand{\LP}{\ensuremath{\Z_{p^k}\left[X,X^{-1}\right]}\xspace}
 
%Denote \LP the set of Laurent polynomials with coefficients over $\Z_{p^k}$. We are
%interested in the degrees of such polynomials both \wrt $X$ and $X^{-1}$.
 
%\subsection{Definizioni e Lemmi di servizio}
In order to study sensitivity of Frobenius LCA over $\Z^n_{p^k}$,  we introduce two concepts about Laurent polynomials. 
\begin{defi}{\blue ($deg^+$ e $deg^-$)}\label{degree}
Given any polynomial $\pp(X)\in\LPK$, the \emph{positive} (resp., \emph{negative}) \emph{degree of $\pp(X)$}, denoted by  $deg^+[\pp(X)]$ (resp., $deg^-[\pp(X)]$) is the maximum (resp., minimum) degree among those of the monomials having both positive (resp., negative) degree and coefficient which is not multiple of $p$. If there is no monomial satisfying both the required conditions, then $deg^+[\pp(X)]=0$ (resp., $deg^-[\pp(X)]$=0).
\end{defi}

\begin{example}
Consider the Laurent polynomial $\pp(X)=4X^{-4}+3X^{-3}+3+7X^{2}+6X^{5}$ with coefficients in  $\Z_8$. Then, $deg^+[\pp(X)]=2$ and $deg^-[\pp(X)]=-3$.
\end{example}


\begin{defi}{\blue (Sensitive polynomial)}\label{polsens}
A polynomial $\pp(X)\in\LPK$ is \emph{sensitive} if either $deg^+[\pp(X)]>0$ or $deg^-[\pp(X)]<0$. 
As a consequence, a Laurent polynomial $\pp(X)$ is not sensitive iff $deg^+[\pp(X)]=deg^-[\pp(X)]=0$.
\end{defi}
Trivially, it is decidable to decide whether a Laurent polynomial is sensitive.
%%
\begin{remark}
Consider a matrix $\M(X)\in\mat{n}{\LPK}$ in Frobenius normal form. The characteristic polynomial of $\M(X)$ is then
%%%
%old
%%%
%\[
%P_{\M}(y)= y^n-c_0(X)-c_1(X) y -\cdots - c_{n-1}(X) y^{n-1}
%\]
%\[
%P_{\M}(y)= 
%PRECEDENTE
%$(-1)^n\left(-\pp_0(X)-\pp_1(X) y -\cdots - \pp_{n-1}(X) y^{n-1} + y^n\right)$\enspace. \\
%$(-1)^n\left(-\pp_1(X)-\pp_2(X) y -\cdots - \pp_{n}(X) y^{n-1} + y^n\right)$\enspace. 
%\]
$\mathscr{P}(y)=(-1)^n\left(-\mm_0(X)-\mm_1(X) y -\cdots - \mm_{n-1}(X) y^{n-1} + y^n\right)$. %\enspace. 
By the Cayley-Hamilton Theorem, one obtains
\begin{eqnarray}\label{cayleyeq}
%OLD \M(X)^n = c_{n-1}(X) M(X)^{n-1} +\dots + c_{1}(X) M(X)^{1} + c_{0}(X) I 
%PRECEDENTI \M^n(X) = \pp_{n-1}(X) \M(X)^{n-1} +\dots + \pp_{1}(X) \M(X)^{1} + \pp_{0}(X) I \enspace.\\
%\M^n(X) = \pp_{n}(X) \M(X)^{n-1} +\dots + \pp_{2}(X) \M(X)^{1} + \pp_{1}(X) I \enspace.
\M^n(X) = \mm_{n-1}(X) \M(X)^{n-1} +\dots + \mm_{1}(X) \M(X)^{1} + \mm_{0}(X) I \enspace.
\end{eqnarray}
\end{remark}
%%
\begin{comment}
The matrix $\M(X)$ of a Frobenius LCA %concentrates %way 
contains too much information for our purposes. %which is not needed 
Hence, we introduce two new matrices that will focus only on the essential information.
\end{comment}
%The matrix $\M(X)$ of a Frobenius LCA %concentrates %way 
%contains too much information for our purposes. %which is not needed 
We now introduce two further matrices that will allows us to access the information hidden inside $\M(X)$.
%
\begin{defi}{\blue ($\U(X)$ e $\LL(X)$)}%{\blue ($\HH_M(X)$ e $\LL_M(X)$)}%{\blue ($\M^{high}(X)$ e $\M^{low}(X)$)}
\label{updown}
For any matrix $\M(X)\in \mat{n}{\LPK}$ in Frobenius normal form %and having  the $n$-th column made of Laurent polynomial $c_0(X), \ldots, c_{n-1}(X)$ with coefficients in $\Z_{p^k}$, 
the matrices %$\M^{high}(X), \M^{low}(X)\in \mat{n}{\LPK}$ 
$\U(X), \LL(X)\in \mat{n}{\LPK}$
associated with $\M(X)$ are the matrices in Frobenius normal %form having  the $n$-th column made of the Laurent polynomial $c^{high}_0(X), \ldots, c^{high}_{n-1}(X)$ and $c^{low}_0(X), \ldots, c^{low}_{n-1}(X)$, 
where each component $\uu_i(X)$ and $\ll_i(X)$ (with $i=0, \ldots, n-1$) of the $n$-th row %$n$-th column %of the vectors 
$\myvec{\uu}(X)$ and $\myvec{\ll}(X)$ of $\U(X)$ and $\LL(X)$, respectively, 
%$\pp^{high}_i(X)$ and $\pp^{low}_i(X)$ of the vectors $\myvec{\pp}^{high}(X)$ and $\myvec{\pp}^{low}(X)$ 
is defined as follows:
%
\begin{comment}
%%%
%OLD
\begin{align*}
c_i^{high}(X)&=
\begin{cases} \text{monomial  of degree } deg^+[c_i(X)] \text{ inside } c_i(X) & \text{if } d_i^+=d^+\\
0 & \text{otherwise}
\end{cases}
\\
c_i^{low}(X)&=
\begin{cases} \text{monomial  of degree } deg^-[c_i(X)] \text{ inside } c_i(X) & \text{if } d_i^-=d^-\\
0 & \text{otherwise}
\end{cases}
\enspace, 
\end{align*}
where $d_i^+=\frac{deg^+[c_i]}{n-i}$, $d_i^-=\frac{deg^-[c_i]}{n-i}$, $d^+=\max\{d_i^+\}$, and $d^-=\min\{d_i^-\}$.
\end{comment}
%%%%
%p
\begin{align*}
\uu_i(X)&=
%\pp_i^{high}(X)&=
\begin{cases} \text{monomial  of degree } deg^+[\mm_i(X)] \text{ inside } \mm_i(X) & \text{if } d_i^+=d^+\\
0 & \text{otherwise}
\end{cases}
\\
%\pp_i^{low}(X)&=
\ll_i(X)&=
\begin{cases} \text{monomial  of degree } deg^-[\mm_i(X)] \text{ inside } \mm_i(X) & \text{if } d_i^-=d^-\\
0 & \text{otherwise}
\end{cases}
\enspace, 
\end{align*}
where $d_i^+=\frac{deg^+[\mm_i(X)]}{n-i}$, $d_i^-=\frac{deg^-[\mm_i(X)]}{n-i}$, $d^+=\max\{d_i^+\}$, and $d^-=\min\{d_i^-\}$.
\end{defi}
%
%%
\begin{example}\label{exupdown} Consider the following matrix $\M(X)\in\mat{4}{\Z_{49}[X,X^{-1}]}$ in Frobenius normal form
\begin{comment}
%PRECEDENTE
\[
\M(X) =\begin{bmatrix}
 0& 0 &0     & X^{-2}+1+X+2X^8 +14X^{123}   \\
 1& 0 &0     & 3 X^{-3}+3+X^2    \\
 0& 1 &0     & 21 X^{-70}+4 X^{-1}+3 X^4    \\
 0& 0 &1     &7 X^{-35}+ X^{-1}+3    \\
 \end{bmatrix} 
\]
\end{comment}
\[
\M(X) =\begin{bmatrix}
 0& 1 &0     & 0   \\
 0& 0 & 1     & 0    \\
 0& 0 &0     & 1    \\
 X^{-2}+1+X+2X^8 +14X^{123} & 3 X^{-3}+3+X^2 & 21X^{-70}+4 X^{-1}+3 X^4     &7 X^{-35}+ X^{-1}+3    \\
 \end{bmatrix} 
\]
We get $d_0^+=2,\ d_1^+=\frac{2}{3},\ d_2^+=2,\ d_3^+=0$ and $d_0^-=-\frac{1}{2},\ d_1^-=-1,\ d_2^-=-\frac{1}{2},\ d_3^-=-1$. Since $d^+=2$ and $d^-=-1$, it holds that $\uu_0(X)=2 X^8,\ \uu_1(X)=0,\ \uu_2(X)=3 X^4,\ \uu_3(X)=0$ and
$\ll_0(X)=0,\ \ll_1(X)=3 X^{-3},\ \ll_2(X)=0,\ \ll_3(X)=X^{-1}$.
%
%$\pp_0^{high}(X)=2 X^8,\ \pp_1^{high}(X)=0,\ \pp_2^{high}(X)=3 X^4,\ \pp_3^{high}(X)=0$ and
%$\pp_0^{low}(X)=0,\ \pp_1^{low}(X)=3 X^{-3},\ \pp_2^{low}(X)=0,\ \pp_3^{low}(X)=X^{-1}$. 
Therefore,
\begin{comment}
%PRECEDENTI
$$\U(X) =\begin{bmatrix}
 0& 0 &0     & 2 X^8    \\
 1& 0 &0     &  0   \\
 0& 1 &0     & 3 X^4    \\
 0& 0 &1     & 0    \\
 \end{bmatrix} 
$$
and
$$\LL(X) =\begin{bmatrix}
 0& 0 &0     & 0    \\
 1& 0 &0     &   3 X^{-3}  \\
 0& 1 &0     & 0    \\
 0& 0 &1     & X^{-1}    \\
 \end{bmatrix} 
$$
\end{comment}
$$\U(X) =\begin{bmatrix}
 0& 1 &0     &0    \\
 0& 0 &1     &  0   \\
 0& 0 &0     & 1    \\
 2 X^8 & 0 & 3 X^4     & 0    \\
 \end{bmatrix} 
$$
and
$$\LL(X) =\begin{bmatrix}
 0& 1 &0     & 0    \\
 0& 0 &1     &   0  \\
 0& 0 &0     & 1    \\
 0& 3 X^{-3} &0     & X^{-1}    \\
 \end{bmatrix} 
$$

\end{example}

\begin{defi}{\blue ($\widehat{\M}$ and $\overline{\M}$)}\label{partevera}
For any Laurent polynomial $\pp(X)\in\LPK$,  %with coefficients in  $\Z_{p^k}$, 
$\widehat{\pp}(X)$ and $\overline{\pp}(X)$ are defined as the Laurent polynomial obtained from $\pp(X)$ by removing all the monomials having coefficients that are multiple of $p$ and $\overline{\pp}(X)= \pp(X)-\widehat{\pp}(X)$, respectively. These definitions extend component-wise to vectors.
For any matrix $\M(X)\in \mat{n}{\LPK}$ in Frobenius normal form, %and having  the $n$-th column made of Laurent polynomial $c_0(X), \ldots, c_{n-1}(X)$ with coefficients in $\Z_{p^k}$, 
$\widehat{\M}(X)$ and $\overline{\M}(X)$ are defined as the matrix obtained from $\M(X)$ by replacing its %$n$-th column $\myvec{\pp}(X)$ with $\hat{\myvec{\pp}}(X)$ 
$n$-th row $\myvec{\mm}(X)$ with $\widehat{\myvec{\mm}}(X)$
and $\overline{\M}(X)=\M(X)-\widehat{\M}(X)$, respectively.
\end{defi}
It is clear that any matrix $\M(X)\in \mat{n}{\LPK}$ in Frobenius normal form can be written as $\M(X)=\widehat{\M}(X) + p \overline{\M'}(X)$, for some $\M'(X)\in \mat{n}{\LPK}$. 
\begin{comment}
Ad esempio se
$p(x)=4x^{-4}+3x^{-3}+3+7x^{2}+6x^{5}$ su $\Z_8$ abbiamo  $\widehat{p(x)}= 3x^{-3}+3+7x^{2} $ e $\overline{p(x)}=4x^{-4} + 6x^{5}$.
\end{comment}


\begin{defi}{\blue (Graph $G_{\M}$)}\label{CH}
Let $\M(X)\in \mat{n}{\LPK}$ be any matrix in Frobenius normal form.  
 The graph $G_{\M}=\langle V_{\M}, E_{\M}\rangle$ associated with $\M(X)$ is such that $V_{\M}=\{1, \ldots, n\}$ and %$E_{\M}=\{(h,k)| \, \M(X)_{(h,k)}\neq 0\}$. 
 $E_{\M}=\{(h,k)\in V^2_{\M} | \, \M(X)^{h}_k \neq 0\}$.
 Moreover, each edge $(h,k)\in E_{\M}$ is labelled with $\M(X)^{h}_k$. %$\M(X)_{(h,k)}$.
 \end{defi}
Clearly, for any matrix $\M(X)\in \mat{n}{\LPK}$ in Frobenius normal form, any natural $t>0$, and any pair $(h,k)$ of entries, the element $\M^t(X)^{h}_k$ is the sum of the weights of all paths of length $t$ starting from $h$ and ending to $k$, where the weight of a path is the product of the labels of its edges.
%%%%%
\begin{example}\label{ex:mat4x4}
Consider any matrix $\M(X)\in\mat{4}{\LPK}$ in Frobenius normal form. The graph $G_{\M}$ associated with $\M(X)$ is represented %can be associated with the graph 
in Figure~\ref{fig:grafo4x4}. It will help to compute $\M^t(X)^{h}_k$.  %$F^i(k,h)$. E' DEFINITO F? SERVE?
Indeed, $\M^t(X)^{h}_k$ is the sum of the labels of all paths of length $t$ from vertex $k$ to $h$ (labels along edges of the same path multiply).
For example for $(h,k)=(4,4)$ one finds
\begin{align*}
\M^1(X)^{4}_4%F^1(4,4)
&=\mm_3(X) \\
\M^2(X)^{4}_4
%F^2(4,4)
&=(\mm_3(X))^2+\mm_2(X)\\
%F^3(4,4)
\M^3(X)^{4}_4
&=\mm_1(X) + 2\mm_2(X)\mm_3(X) + (\mm_3(X))^3\\
\end{align*}
and so on.
\begin{comment}
%%VECCHIO con p_0...
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
\tikzset{edge/.style = {->,> = latex'}}
% vertices
\node[vertex] (c0) at  (0,0) {$1$};
\node[vertex] (c1) at (2,0) {$2$};
\node[vertex] (c2) at (4,0) {$3$};
\node[vertex] (c3) at  (2,2) {$4$};
%\node [shape=circle,minimum size=1.5em] (a3) at (4.5,0) {q};
%\node [vertex] (cn1) at (6.5,0) {$c_{n-1}$};
%edges
\draw[edge] (c0)  to[bend left]  node[left] {$\pp_0(X)$} (c3)  ;
\draw[edge] (c1) to[bend left] node[below] {1} (c0);
\draw[edge] (c1) to[bend left] node[left] {$\pp_1(X)$} (c3);
\draw[edge] (c2) to[bend left] node[below] {1} (c1);
\draw[edge] (c2) to[bend left] node[right] {$\pp_2(X)$} (c3);
\draw[edge] (c3) to[bend left] node[above] {1} (c2);
\draw[edge] (c3) to[loop]  node[above]  {$\pp_3(X)$} (c3); 
%\path (c2) to node {\dots} (c3) ;
\end{tikzpicture}
\end{center}
\caption{Graph $G_{\M}$ associated with $\M(X)$ from Example~\ref{ex:mat4x4}.}
\label{fig:grafo4x4}
\end{figure}
\end{comment}
%%%%
\begin{comment}
%grafo matrice colonna
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
\tikzset{edge/.style = {->,> = latex'}}
% vertices
\node[vertex] (c0) at  (0,0) {$1$};
\node[vertex] (c1) at (2,0) {$2$};
\node[vertex] (c2) at (4,0) {$3$};
\node[vertex] (c3) at  (2,2) {$4$};
%\node [shape=circle,minimum size=1.5em] (a3) at (4.5,0) {q};
%\node [vertex] (cn1) at (6.5,0) {$c_{n-1}$};
%edges
\draw[edge] (c0)  to[bend left]  node[left] {$\mm_0(X)$} (c3)  ;
\draw[edge] (c1) to[bend left] node[below] {1} (c0);
\draw[edge] (c1) to[bend left] node[left] {$\mm_1(X)$} (c3);
\draw[edge] (c2) to[bend left] node[below] {1} (c1);
\draw[edge] (c2) to[bend left] node[right] {$\mm_2(X)$} (c3);
\draw[edge] (c3) to[bend left] node[above] {1} (c2);
\draw[edge] (c3) to[loop]  node[above]  {$\mm_3(X)$} (c3); 
%\path (c2) to node {\dots} (c3) ;
\end{tikzpicture}
\end{center}
\caption{Graph $G_{\M}$ associated with $\M(X)$ from Example~\ref{ex:mat4x4}.}
\label{fig:grafo4x4}
\end{figure}
\end{comment}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
\tikzset{edge/.style = {->,> = latex'}}
% vertices
\node[vertex] (c0) at  (0,0) {$1$};
\node[vertex] (c1) at (2,0) {$2$};
\node[vertex] (c2) at (4,0) {$3$};
\node[vertex] (c3) at  (2,2) {$4$};
%\node [shape=circle,minimum size=1.5em] (a3) at (4.5,0) {q};
%\node [vertex] (cn1) at (6.5,0) {$c_{n-1}$};
%edges
\draw[edge] (c3)  to[bend right]  node[left] {$\mm_0(X)$} (c0)  ;
\draw[edge] (c0) to[bend right] node[below] {1} (c1);
\draw[edge] (c3) to[bend right] node[left] {$\mm_1(X)$} (c1);
\draw[edge] (c1) to[bend right] node[below] {1} (c2);
\draw[edge] (c3) to[bend right] node[right] {$\mm_2(X)$} (c2);
\draw[edge] (c2) to[bend right] node[above] {1} (c3);
\draw[edge] (c3) to[loop]  node[above]  {$\mm_3(X)$} (c3); 
%\path (c2) to node {\dots} (c3) ;
\end{tikzpicture}
\end{center}
\caption{Graph $G_{\M}$ associated with $\M(X)$ from Example~\ref{ex:mat4x4}.}
\label{fig:grafo4x4}
\end{figure}
\end{example}
%%%%
  %\emph{p} $p$ \textit{p} 
%$\mathbbm{p}$ 
%$\mathbbmss{p}$ %$\mathbbmtt{p}$ 
%
%
\begin{lemma}\label{piup}
Let $p>1$ be a prime number and $a, b\geq 0$, $k>0$ be integers such that $1\leq a < p^k$ and $\gcd(a,p)= 1$. Then,
\begin{equation}\label{lemmapiup}
\modulo{a+p b}{p^k}\neq 0
\end{equation}
\end{lemma}
\begin{proof}
For the sake of argument, assume that  $\modulo{a+p  b}{p^k} = 0$. Thus, $a+p  b= c  p^k$ for some $c\geq 0$ and then $a= c  p^k - p b = p(c  p^{k-1}-b )$, that contradicts $\gcd(a,p)= 1$.\qed
\end{proof}

\begin{lemma}\label{fiboext}
Let $p>1$ be a prime number and $h,k$ be two positive integers. Let $l_1,\dots,l_h$  and $\alpha_1,\dots,\alpha_h$ be positive integers such that $l_1<l_2<\cdots <l_h$ and for each $i=1, \ldots, h$ both  $1\leq \alpha_i< p^k$  and $\gcd(\alpha_i,p)=1$ hold. Consider the sequence $b:\Z\to\Z_{p^k}$ defined for any $l\in\Z$ as
\begin{eqnarray}\label{eq1}
b_l&=&\modulo{\alpha_1 b_{l-l_1}+\cdots + \alpha_h b_{l-l_h}}{p^k} \quad \text{ if } l>0\\
\nonumber
b_0&=&1\\
\nonumber
b_l&=&0\quad\text{ if } l<0
\end{eqnarray}
Then, it holds that $\modulo{b_l}{p} \neq 0$ for infinitely many $l\in\N$.
\end{lemma}
\begin{proof}
Set $dz=\left |\{ l\in\N : \modulo{b_l}{p} \neq 0 \}\right |$. For the sake of argument, assume that $dz$ is finite. Then, there exists $h_0\in\N$ such that $\modulo{b_{h_0}}{p} \neq 0$ and $\modulo{b_{l}}{p} = 0$ for all $l>h_0$. Thus, there exist non negative integers $s_0, s_1, \ldots, s_{h-1}$ such that  $b_{l_h+h_0}=ps_0$ and $b_{l_h+h_0-l_i}=ps_i$ for each $i=1, \ldots, h-1$. Equation~\eqref{eq1}  can be rewritten with $l=l_h+h_0$ as 
\begin{equation*}\label{eq2}
b_{l_h+h_0}=\modulo{\alpha_1b_{l_h+h_0-l_1}+\cdots + \alpha_{h-1} b_{l_h +h_0 - l_{h-1}} + \alpha_h b_{h_0}}{p^k}\enspace,
\end{equation*}
which gives 
\begin{equation*}\label{eq2}
ps_0=\modulo{\alpha_1ps_1+\cdots + \alpha_{h-1} ps_{h-1} + \alpha_h b_{h_0}}{p^k}\enspace.
\end{equation*}
Thus, there  must exist an integer $s\geq 0$ such that
%%%
\begin{equation*}\label{eq2}
%\alpha_1ps_1+\cdots + \alpha_{h-1} ps_{h-1} + \alpha_h b_{h_0}=
 p\sum_{i=1}^{h-1} \alpha_i s_i  + \alpha_h b_{h_0} =s p^k + ps_0\enspace,
\end{equation*}
or, equivalently,
\begin{equation*}\label{eq2}
%\alpha_1ps_1+\cdots + \alpha_{h-1} ps_{h-1} + \alpha_h b_{h_0}=
  \alpha_h b_{h_0} =p\left ( s p^{k-1} + s_0 - \sum_{i=1}^{h-1} \alpha_i s_i \right ) \enspace,
\end{equation*}
with $ps_0 < p^k$. If $s p^{k-1} + s_0 - \sum_{i=1}^{h-1} \alpha_i s_i =0$, we get  $\alpha_h b_{h_0}=0$ that contradicts either the assumption $\modulo{b_{h_0}}{p} \neq 0$ or the hypothesis $1\leq \alpha_h< p^k$. Otherwise, $p$ must divide either $\alpha_h$ or $b_{h_0}$. However, that is impossible since $\gcd(\alpha_h,p)=1$ and $\gcd(b_{h_0},p)=1$.
\begin{comment}
\begin{equation*}\label{eq3}
p s=\modulo{\alpha_h b_{h_0}}{p^k}
\end{equation*}
As a consequence, $p$ divides either $\alpha_h$ or $b_{h_0}$. However, that is impossible since $\gcd(\alpha_h,p)=1$ and $\gcd(b_{h_0},p)=1$.
\end{comment}
%%%
\qed 
\end{proof}

For any matrix $\M(X)\in\mat{n}{\LPK}$ in Frobenius normal form, we are now going to study the behavior of $\U^{t}(X)$ and $\LL^{t}(X)$, and, in particular, of their elements $\U^{t}(X)^n_n$ and $\LL^{t}(X)^n_n$. These will turn out to be crucial in order to establish the sensitivity of the LCA defined by $\M(X)$.
To make our arguments clearer we prefer to start with an example.

\begin{ex}\label{monex}
Consider the following matrix $\M(X)\in\mat{4}{\Z_{49}[X,X^{-1}]}$ in Frobenius normal form
\begin{comment}
%PRECDENTE COLONNA
\[
\M(X) =\begin{bmatrix}
 0& 0 &0    & X^{-2}+1+X+16X^6    \\
 1& 0 &0    & 13 X^{-3}+3+X^2    \\
 0& 1 &0    & 34 X^{-1}+8 X^3    \\
 0& 0 &1    & X^{-1}+31    \\
 \end{bmatrix} 
 \in\mat{4}{\Z_{49}[X,X^{-1}]}
\]
\end{comment}
\[
\M(X) =\begin{bmatrix}
 0& 1 &0    &    0 \\
 0& 0 &1   & 0    \\
 0& 0 &0    &  1    \\
 X^{-2}+1+X+16X^6& 13 X^{-3}+3+X^2 &34 X^{-1}+8 X^3    & X^{-1}+31    \\
 \end{bmatrix} 
 \in\mat{4}{\Z_{49}[X,X^{-1}]}
\]
%From the definitions 
One finds $d^+=3/2$ and then
\begin{comment}
%precedente colonna
\[
\U(X) =\begin{bmatrix}
 0& 0 &0     & 16 X^6    \\
 1& 0 &0     &  0   \\
 0& 1 &0     & 8 X^3    \\
 0& 0 &1     & 0    \\
 \end{bmatrix} 
\]
\end{comment}
\[
\U(X) =\begin{bmatrix}
 0& 1 &0     & 0    \\
 0& 0 &1     &  0   \\
 0& 0 &0     & 1    \\
 16 X^6& 0 & 8 X^3 & 0    \\
 \end{bmatrix} 
\]
The graph $G_{\U}$ is represented in Figure~\ref{fig:monex}.
%
\begin{comment}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
\tikzset{edge/.style = {->,> = latex'}}
% vertices
\node[vertex] (c0) at  (0,0) {$1$};
\node[vertex] (c1) at (2,0) {$2$};
\node[vertex] (c2) at (4,0) {$3$};
\node[vertex] (c3) at  (2,2) {$4$};
\draw[edge] (c0)  to[bend left]  node[left] {$16X^6$} (c3)  ;
\draw[edge] (c1) to[bend left] node[below] {1} (c0);
\draw[edge] (c2) to[bend left] node[below] {1} (c1);
\draw[edge] (c2) to[bend left] node[near end,left] {$8X^3$} (c3);
\draw[edge] (c3) to[bend left] node[above] {1} (c2);
\end{tikzpicture}
\end{center}
\caption{The graph $G_{\U}$ from Example~\ref{monex}.}
\label{fig:monex}
\end{figure}
\end{comment}
\begin{figure}[htb]
\begin{center}
\begin{tikzpicture}
\tikzset{vertex/.style = {shape=circle,draw,minimum size=1.5em}}
\tikzset{edge/.style = {->,> = latex'}}
% vertices
\node[vertex] (c0) at  (0,0) {$1$};
\node[vertex] (c1) at (2,0) {$2$};
\node[vertex] (c2) at (4,0) {$3$};
\node[vertex] (c3) at  (2,2) {$4$};
\draw[edge] (c3)  to[bend right]  node[left] {$16X^6$} (c0)  ;
\draw[edge] (c0) to[bend right] node[below] {1} (c1);
\draw[edge] (c1) to[bend right] node[below] {1} (c2);
\draw[edge] (c3) to[bend right] node[left] {$8X^3$} (c2);
\draw[edge] (c2) to[bend right] node[above] {1} (c3);
\end{tikzpicture}
\end{center}
\caption{The graph $G_{\U}$ from Example~\ref{monex}.}
\label{fig:monex}
\end{figure}
The values $\U^t(X)^4_4$, $\modulo{\U^t(X)^4_4}{49}$, and $td^+$, for $t=1, \ldots,  8$, are listed below.
\begin{center}
\begin{tabular}{|c|c|c|c|}
\hline
  & $\U^t(X)^4_4$ & $\modulo{\U^t(X)^4_4}{49}$&$td^+$ \\
\hline
$t=1$ & $0$ & $0$ &$3/2$\\
$t=2$ & $8X^3$ & $8X^3$&$3$  \\
$t=3$ & $0$ & $0$ &$9/2$\\
$t=4$ & $80X^6$  & $31X^6$ &$6$\\
$t=5$ & $0$ & $0$ &$15/2$\\
$t=6$ & $768X^9$ & $33X^9$ &$9$\\
$t=7$ & $0$ & $0$&$21/2$ \\
$t=8$ & $7424 X^{12}$ & $25X^{12}$&$12$ \\
\hline
\end{tabular}
\end{center}
\end{ex}
\begin{notation}
For a sake of simplicity, for any given matrix $\M(X)\in\mat{n}{\LPK}$ in Frobenius normal form, from now on we will denote by  $\uu^{(t)}(X)$ and $\ll^{(t)}(X)$ the elements $(\U^t(X))_{n}^n$ and $\LL^{t}(X)^n_n$, respectively. %$\M^{high}(X)_{(n,n)}^m$
\end{notation}
\begin{lemma}\label{sempremonomio}
Let $\M(X)\in \mat{n}{\LPK}$ be a matrix such that $\M(X)=\widehat{\NN}(X)$ for some matrix $\NN(X) \in \mat{n}{\LPK}$ in Frobenius normal form. 
For any natural $t>0$, $\uu^{(t)}(X)$ (resp., $\ll^{(t)}(X)$) is either null or a monomial of degree $td^+$ (resp., $td^-$). %or $(\U^t(X))_{n}^n=0$.  
\begin{comment}
Sia $F$ una matrice $n\times n$ di Frobenius su $\Z_{p^k}$ depurata da monomi con coefficienti multipli di $p$.
Assumiamo che $d^+>0$. Allora $(F^{high})^m(n,n)$ \`e un monomio di grado $md^+$ oppure \`e uguale a $zero$
\end{comment}
\end{lemma}
\begin{proof} 
We show that the statement is true for $\uu^{(t)}(X)$ (the proof concerning $\ll^{(t)}(X)$ is identical by replacing $d^+$, $\U(X)$ and related elements with $d^-$, $\LL(X)$ and related elements). For  each $i\in V_{\U}$, let $\gamma_i$ be the simple cycle of $G_{\U}$ from $n$ to $n$ and passing  through the edge $(n,i)$. Clearly, $\gamma_i$ is the path $n\to i\to i+1\ldots\to n-1\to n$ (with $\gamma_n$ the self-loop $n\to n$) of length $n-i+1$ and its weight is the monomial $\uu_{i-1}(X)$ of degree $(n-i+1)d^+$. We know that $\uu^{(t)}(X)$ is the sum of the weights of all cycles of length $t$ starting from $n$ and ending to $n$ in $G_{\U}$ if at least one of such cycles exists, $0$, otherwise. In the former case, each of these cycles can be  decomposed in a certain number $s\geq 1$ of simple cycles $\gamma_{j_1}^1,\ldots, \gamma_{j_s}^s$ of lengths giving sum $t$, \ie,  such that $\sum_{i=1}^{s} (n-j_i+1) = t$. Therefore, $(\U^t(X))_{n}^n$ is a monomial of degree $\sum_{i=1}^{s} (n-j_i+1)d^+ = t d^+$.\qed
\end{proof}
\begin{comment}
\begin{proof} DA SISTEMARE
For simplicity sake, let $\M=\M^{high}(X)$.
Remark that a simple cycle of $G_{\M}$ starting at $n$ and ending in $n$ has always the same form
$n\to n-1\to\ldots\to i\to n$ and its length is $n-i$ for some $i\in[1,n]$. Call $S_i$ the simple cycle passing through the edge $(i,n)$.
The product of labels of the simple cycle $S_i$ is the monomial
$c_i(X)$ of degree $d_i$ (recall the definition of $\M^{high}$). Now consider $\M^m_{(n,n)}$. If there is no cycle of lenght $m$ in $G_{\M}$
then $\M^m_{(n,n)}=0$ and we are done. If there exists at least a cycle of length $m$, we claim that the value found at position 
$(n,n)$ is a monomial of degree $md^+$ or the constant value $0$. Indeed, the value found is the sum of the contributions of all 
possible cycles of length $m$
starting at $n$ and ending in $n$. Consider any of such cycles $S$. It can be decomposed into elementary cycles such that
\begin{align}\label{eq:decomposizione-di-m}
m=\sum_{i=1}^{n}k_i|S_i|=\sum_{i=1}^{n}k_i(n-i)
\end{align}
for suitable coefficients $k_i$ which indicate the number of times that the simple cycle $S_i$ is taken. Each $S_i$ (taken with its multiplicity) will contribute a monomial of degree $k_id_i$. Therefore, the degree of the monomial
associated with $S$ is $\sum_{i=1}^{n}k_id_i$ (recall that the product of labels of the cycle is taken). Recall that, by Definition~\ref{updown}, $d_i=d^+(n-i)$. Therefore, $\sum_{i=1}^{n}k_id_i=\sum_{i=1}^{n}k_id^+(n-i)=d^+\sum_{i=1}^{n}k_i(n-i)=md^+$, where in last equality
we used the decomposition of $m$ given in~\eqref{eq:decomposizione-di-m}. Since all cycles of length $m$ will contribute
a monomial of degree $md^+$ then either the sum of the coefficients is 0 modulo $p^k$ or it produces a single monomial
of degree $md^+$.\qed
\end{proof}
\end{comment}
%DUBBIO NEL SEGUENTE: PERCHE' SI USANO I COEFFICIENTI (POLINOMI) DI M E NON DI U??
\begin{lemma}\label{tdim}
Let $\M(X)\in\mat{n}{\LPK}$
be any matrix in Frobenius normal form.
For every integer $t\geq 1$ both the following recurrences hold %Si noti che $F^0=I$.
%%%%
\begin{comment}
\begin{eqnarray}\label{eqgen1}
\uu^{(t)}(X) &=&  %c_{n-1}(X)V(m-1)+ \cdots + c_{1}(X)V(m-n+1)+  c_0 V(m-n)(X)
\mm_{n-1}(X)\uu^{(t-1)}(X)+ \cdots + \mm_{1}(X)\uu^{(t-n+1)}(X) +  \mm_0(X)\uu^{(t-n)}(X) 
\end{eqnarray}
\end{comment}
%%%%%
\begin{eqnarray}\label{eqgen1}
\uu^{(t)}(X) &=&  %c_{n-1}(X)V(m-1)+ \cdots + c_{1}(X)V(m-n+1)+  c_0 V(m-n)(X)
\uu_{n-1}(X)\uu^{(t-1)}(X)+ \cdots + \uu_{1}(X)\uu^{(t-n+1)}(X)+  \uu_0(X)\uu^{(t-n)}(X)\\
\ll^{(t)}(X) &=&  %c_{n-1}(X)V(m-1)+ \cdots + c_{1}(X)V(m-n+1)+  c_0 V(m-n)(X)
\ll_{n-1}(X)\ll^{(t-1)}(X)+ \cdots + \ll_{1}(X)\ll^{(t-n+1)}(X)+  \ll_0(X)\ll^{(t-n)}(X)
\end{eqnarray}
with the related initial conditions 
\begin{eqnarray}
\uu^{(0)}(X) &=& 1, \quad \ll^{(0)}(X) = 1\label{eqgen2a} \\ 
\uu^{(l)}(X) &=&0, \quad \ll^{(l)}(X) =0\quad \text{for $l<0$.} 
\label{eqgen2b}
\end{eqnarray}
\end{lemma}
\begin{proof}
We show the recurrence involving $\uu^{(t)}(X)$ (the proof for $\ll^{(t)}(X)$ is identical by replacing $\U(X)$ and its elements with $\LL(X)$ and its elements). Since $\U(X)$ is in Frobenius normal form too, by~\eqref{cayleyeq}, Recurrence~\eqref{eqgen1} holds for every $t\geq n$. It is clear that $\uu^{(0)}(X)=1$. Furthermore, by the structure of the graph $G_{\U}$ and the meaning of $\U(X)^n_{n}$, Equation~\eqref{eqgen1} is true under the initial conditions~\eqref{eqgen2a} and~\eqref{eqgen2b} for each $t=1, \ldots, n-1$.
\qed
\end{proof}

\begin{lemma}\label{infinitim}
Let $\M(X)\in \mat{n}{\LPK}$ be a matrix such that $\M(X)=\widehat{\NN}(X)$ for some matrix $\NN(X) \in \mat{n}{\LPK}$ in Frobenius normal form. Let $\upsilon(t)$ (resp., $\lambda(t)$) be the coefficient of $\uu^{(t)}(X)$ (resp., $\ll^{(t)}(X)$). It holds that $\gcd[\upsilon(t),p]=1$ (resp., $\gcd[\upsilon(t),p]=1$),  for infinitely many $t\in\N$. 
\\
In particular, if the value  $d^+$ (resp.,  $d^-$) associated with $\M(X)$ is non null, then for infinitely many $t\in\N$ both $\modulo{\uu^{(t)}(X)}{p^k}\neq 0$ and $deg(\modulo{\uu^{(t)}(X)}{p^k})\neq 0$ (resp., $\modulo{\ll^{(t)}(X)}{p^k}\neq 0$ and $deg(\modulo{\ll^{(t)}(X)}{p^k})\neq 0$) hold. 
In other terms, if $d^+>0$ (resp.,  $d^-<0$) then $|\{\uu^{(t)}(X), t\geq 1\}|=%|\{\U^t(X), t\geq 1\}|
\infty$ (resp., $|\{\ll^{t}(X), t\geq 1\}|%=|\{\LL^t(X), t\geq 1\}|
=\infty$).%, and in that case we say that $\U^t(X)$ diverges (resp., $\LL^t(X)$ diverges).
\end{lemma}
\begin{proof}
%Let $\upsilon(t)$ be the coefficient of $u(t)$. 
We show the statements concerning $\upsilon(t)$, $\U(X)$, $\uu^{(t)}(X)$, and $d^+$. %Assume that $d^+>0$ and 
Replace $X$ by $1$ in the matrix $\U(X)$. Now, the coefficient $\upsilon(t)$ is just the element of position $(n,n)$ in the $t$-th power of the obtained matrix $\U(1)$. Over $\U(1)$, the thesis of Lemma~\ref{tdim} is still valid replacing $\uu^{(t)}(X)$ by $\upsilon(t)$. Thus, for every $t\in\N$
%%%%%
\begin{comment}
\begin{eqnarray}
\upsilon(t) &=&  c_{n-1}\upsilon(t-1)+ \cdots +  c_1 \upsilon(t-n+1)+c_0 \upsilon(t-n)\\
\end{eqnarray}
\end{comment}
%%%%%
\begin{eqnarray*}
\upsilon(t) &=&  \uu_{n-1}(1)\upsilon(t-1)+ \cdots +  \uu_1(1) \upsilon(t-n+1)+\uu_0(1) \upsilon(t-n)
\end{eqnarray*}
with initial conditions
\begin{eqnarray*}\label{eqgen3}
\upsilon(0)&=& 1 \\
\upsilon(l)&=&0\quad \text{for $l<0$,}
\end{eqnarray*}
where each $\uu_i(1)$ is the coefficient of the monomial $\uu_i(X)$ inside $\U(X)$. Thus, it follows that 
\begin{equation*}\label{eq55}
\modulo{\upsilon(t)}{p^k} = 
\modulo{\uu_{n-1}(1)\upsilon(t-1)+ \cdots +  \uu_1(1) \upsilon(t-n+1)+\uu_0(1) \upsilon(t-n)}{p^k}
\end{equation*}
By Lemma~\ref{fiboext} we obtain that $\gcd[\upsilon(t),p]=1$ (and so $\modulo{\upsilon{(t)}}{p^k}\neq 0$, too) for infinitely many $t\in\N$. In particular, if the value  $d^+$ associated with $\M(X)$ is non null, then, by the structure of $G_{\U}$ and Lemma~\ref{sempremonomio},  both $\modulo{\uu^{(t)}(X)}{p^k}\neq 0$ and $deg(\modulo{\uu^{(t)}(X)}{p^k})\neq 0$ hold
for infinitely many $t\in\N$, too. Therefore, $|\{\uu^{(t)}(X), t\geq 1\}|=%|\{\U^t(X), t\geq 1\}|=
\infty$. The same proof runs for the statements involving $\lambda(t)$, $\LL(X)$, $\uu^{(t)}(X)$, and $d^-$ provided that these replace $\upsilon(t)$, $\U(X)$, $\uu^{(t)}(X)$, and $d^+$, respectively.%, and one assumes $d^-<0$ instead of $d^+>0$. 
\qed
\end{proof}
\begin{comment}
As an immediate consequence of Lemma~\ref{infinitim} one obtains the following.

\begin{teo}\label{union}
Let $\M(X)\in \mat{n}{\LPK}$ be a matrix such that $\M(X)=\widehat{\NN(X)}$ for some matrix $\NN(X) \in \mat{n}{\LPK}$ in Frobenius normal form. If the value  $d^+$ associated with $\M(X)$ is non null, then for infinitely many $t\in\N$ it holds that $deg(\modulo{\uu^{(t)}(X)}{p})\neq 0$ and then
$$deg(\modulo{\uu^{(t)}(X)}{p^k})\neq 0\enspace, $$ ERA MODULO P
or, equivalently, $|\{\U^t(X), t\geq 1\}|=\infty$ (\ie, in other words, $\U^t(X)$ diverges).
\end{teo}
\end{comment}
The following Lemma puts in relation the behavior of $\uu^{(t)}(X)$ or $\ll^{(t)}(X)$ with that of $\widehat{\M}^{\, t}(X)_n^n$, 
%divergence of $\U^t(X)$ or $\LL^t(X)$ with that of $\widehat{\M}^{\, t}(X)$, 
for any matrix $\M(X)\in \mat{n}{\LPK}$  in Frobenius normal form. 
\begin{lemma}\label{corollario}
Let $\M(X)\in \mat{n}{\LPK}$ be a matrix in Frobenius normal form. 
\begin{comment}
If $|\{\U^t(X), t\geq 1\}|=\infty$ (\ie, $\U^t(X)$ diverges) then $|\{\widehat{\M}^{\, t}(X), t\geq 1\}|=\infty$ (\ie, $\widehat{\M}^{\, t}(X)$ also diverges).
\end{comment}
If either $|\{\uu^{(t)}(X), t\geq 1\}|=\infty$ or $|\{\ll^{(t)}(X), t\geq 1\}|=\infty$ %(that implies that $\U^t(X)$ diverges) 
then $|\{\widehat{\M}^{\, t}(X)_n^n, t\geq 1\}|=\infty$.
%(that implies that $|\{\widehat{\M}^{\, t}(X), t\geq 1\}|=\infty$, \ie, $\widehat{\M}^{\, t}(X)$ also diverges).
\begin{comment}
DOMANDA
$|\{\uu^t(X), t\geq 1\}|=\infty$ SE E SOLO SE $|\{\U^t(X), t\geq 1\}|=\infty$??
\\

$|\{\widehat{\M}^{\, t}(X)_n^n, t\geq 1\}|=\infty$ SE E SOLO SE $\widehat{\M}^{\, t}(X)$??
\end{comment}
\end{lemma}
%
\begin{proof}
Assume that $|\{\uu^{(t)}(X), t\geq 1\}|=\infty$. Since $G_{\U}$ is a subgraph of $G_{\widehat{\M}}$ (with different labels), for each integer $t$ from Lemma~\ref{infinitim} applied to $\widehat{\M}(X)$, the cycles of length $t$ in $G_{\widehat{\M}}$ with weight containing a monomial of degree $td^+$ are exactly the cycles of length $t$ in $G_{\U}$. Therefore, it follows that $|\{\widehat{\M}^{\, t}(X)_n^n, t\geq 1\}|=\infty$. The same argument on $G_{\LL}$ and involving $d^-$ allows to prove the thesis if $|\{\ll^{(t)}(X), t\geq 1\}|=\infty$.
\begin{comment}
\\

Remark that given a matrix 
$\M(X)\in \mat{n}{\LP}$ in Frobenius normal form in which the coefficients of  the Laurent polynomials are not multiple of $p$, the infinite
set of values in Lemma~\ref{infinitim} for which there exists a cycle from $n$ to $n$ in $G_{\M^{high}}$ is a subset of the values
for which there exists a cycle from $n$ to $n$ in $G_{\M}$ since $G_{\M^{high}}$ is a subgraph of $G_{\M}$. Indeed, the following result holds.
\end{comment}
\end{proof}
\begin{comment}
Using the comment just after Definition~\ref{partevera} and the additivity property, one can easily prove the following result.
\end{comment}
\begin{comment}
By Definition~\ref{partevera}, one can easily prove the following result. TOGLIERE
\begin{lemma}\label{spezzan}
Let $\M(X)\in \mat{n}{\LPK}$ be a matrix in Frobenius normal form. 
%Sia $F$ una matrice di Frobenius $n\times n$ (ultima colonna formata dai polinomi $c_i$ di Laurent su $\Z_{p^k}$, $p$ primo, $k\geq 1$).
%Allora per qualsiasi $n\geq 1$ esiste $M$ matrice $n\times n$ con elementi polinomi di Laurent su $\Z_{p^k}$ tale che
Then, for any integer $t>0$, there exists a matrix $\M'(X)\in \mat{n}{\LPK}$ such that
\begin{equation}\label{spezzon}
\M^t(X)=\widehat{\M}^t(X) + p\M'(X)
\end{equation}
\end{lemma}
\end{comment}
%%%%%%%
\begin{comment}
\begin{teo}\label{th:uno}
Consider a matrix $\M(X)\in \mat{n}{\LPK}$ in Frobenius normal form and let $F$ be the corresponding CA.
The following statements are equivalent:
\begin{enumerate}
\item $F$ is sensitive to initial conditions;
\item
$\limsup_{t\to\infty} deg[\M(X)^t]= \infty$;
\item
$|\{ \M(X)^i,\ i\geq 1 \}|=\infty$;
\item $F$ is not equicontinuous.
\end{enumerate}
\end{teo}
\begin{proof}
It is pretty clear that items $2.$ and $3.$ are equivalent. The equivalence between items $1.$ and $4.$ is a simple consequence of the
additivity of $F$ and the Knudsen's lemma. Finally, assume that $3.$ is false, then it is clear that $F$ is equicontinuous that is to say
that $4.$ is false.\qed
\end{proof}
\end{comment}

\begin{comment}
\begin{teo}\label{frobeniusSensitivity}
Consider a matrix $\M(X)\in \mat{n}{\LPK}$ in Frobenius normal form
and let $\myvec{c}$ be its $n$-th vector.
The LCA associated with $\M$ is sensitive to initial conditions
if and only if $\myvec{c}_i$ is sensitive for some $i\in[0,n)$.
\end{teo}
\end{comment}
We are now able to present and prove the main result of this section. It shows a decidable characterization of sensitivity for Frobenius LCA over $\Z_{p^k}^n$.
\begin{lemma}\label{frobeniusSensitivity}
Let $\left ( (\Z_{p^k}^n)^{\Z}, F \right)$ be any Frobenius LCA over $\Z_{p^k}^n$ and let $(\mm_0(X), \ldots, \mm_{n-1})$ be the $n$-th row of the matrix $\M(X)\in\mat{n}{\LPK}$ in Frobenius normal form associated with $F$. Then, $F$ is sensitive to the initial conditions if and only if $\mm_i(X)$ is sensitive for some $i\in[0,n-1]$.
\end{lemma}
%%%%
\begin{proof}
Let us prove the two implications separately.
\\
Assume that all $\mm_i(X)$ are not sensitive. Then, $\widehat{\M}(X)\in \mat{n}{\Z_{p^k}}$, \ie, it does not contain the formal variable $X$, and $\M(X)=\widehat{\M}(X)+p\M'(X)$, for some $\M'(X)\in\mat{n}{\LPK}$ in Frobenius normal form. Therefore, for any integer $t>0$, $\M^t(X)$ is the sum of terms, each of them consisting of a product in which $p^j$ appears as factor, for some natural $j$ depending on $t$ and on the specific term which $p^j$ belongs to. Since every element of $\M^t(X)$ is taken modulo $p^k$, for any natural $t>0$ it holds that in each term of such a sum $p^j$ appears with $j\in[0, k-1]$ (we stress that $j$ may depend on $t$ and on the specific term of the sum, but it is always bounded by $k$). Therefore, $|\{\M^i(X): i>0\}|<\infty$ and so, by Proposition~\ref{prop:dich}, $F$ is not sensitive to the initial conditions.

Conversely, suppose that $\mm_i(X)$ is sensitive for some $i\in[0,n-1]$ and $d^+>0$ (the case $d^-<0$ is identical). By Definition~\ref{partevera}, for any natural $t>0$ there exists a matrix $\M'(X)\in \mat{n}{\LPK}$ such that $\M^t(X)=\widehat{\M}^t(X) + p\M'(X)$. %IL FATTO CHE $M'$ DIPENDE DA $t$ E' UN PROBLEMA? 
By a combination of Lemmata~\ref{infinitim} and~\ref{corollario}, we get $|\{\widehat{\M}^{\, t}(X)_n^n, t\geq 1\}|=\infty$ and so, by  Lemma~\ref{piup}, $|\{\M^t(X)_n^n, t\geq 1\}|=\infty$ too. Therefore, it follows that $|\{\M^t(X), t\geq 1\}|=\infty$ and, by Proposition~\ref{prop:dich}, we conclude that $F$ is sensitive to the initial conditions.
%$\widehat{\M}^t(X)$ diverges and, in particular, its element $\widehat{\M}^t(X)^n_n$. %BISOGNEREBBE PARLARE DELL' ELEMENTO RIGA $n$ COLONNA $n$ SIA QUI CHE NEI LEMMI (NEL PRIMO OK NEL SECONDO NO). 
%Thus, by  Lemma~\ref{piup}, $\M^t(X)_n^n$ diverges too, and, by Proposition~\ref{prop:dich}, we conclude that $F$ is sensitive to the initial conditions.
\qed
\end{proof}
\begin{comment}
\begin{proof}
\noindent
Let us prove that $F$ sensitive to initial conditions $\Longrightarrow$ there exists at least a sensitive polynomial $\myvec{c}_i(X)$.\\
Assume that $F$ sensitive to initial conditions and the associated matrix $\M$ is Frobenius normal form but $\M$ does not contain any
sensitive polynomial. This means that $f$ only depends on the central variable, namely
$f(\myvec{x}_{i-r},\ldots,\myvec{x}_i,\ldots,\myvec{x_{i+r}})=\M_0\myvec{x}_i$. By Knusden's lemma, we can focus on finite configurations
\ie configurations for which only a finite number of sites contain a non-null vector. Let us prove that $\myvec{0}$ (the configuration
containing only null vectors) is an equicontinuous point. Indeed, for any $\varepsilon>0$, choose $\delta=\epsilon/2$. Then, for any
$\myvec{x}\in B_{\delta}(\myvec{0})$, it is clear that $\forall m\in\N,\,d(F^m(\myvec{0}),F^m(\myvec{x}))=d(\myvec{0},F^m(\myvec{x}))<\delta$. Hence, $F$ is not sensitive to initial conditions contradicting the initial hypothesis.

Let us prove that if there exists $i\in[0,n)$ such that $\myvec{c}_i(X)$ is sensitive $\Rightarrow F$ is sensitive.
By Lemma~\ref{spezzan}, it holds that $\M^m=\widehat{\M}^m + p \M'$ and the combination of Theorems~\ref{union} and \ref{corollario},
$\widehat{\M}^m$ diverges.
Since the element $\M^m_{(n,n)}$ is the sum of $\widehat{\M}^m_{(n,n)}$ and $p \M'_{(n,n)}$ and $\widehat{\M}^m_{(n,n)}$, by  Lemma~\ref{piup}
we conclude that $F^m_{(n,n)}$ diverges too. Theorem~\ref{th:uno} allows to conclude.
\qed
\end{proof}
\end{comment}
%%%%
\begin{comment}
\ignora{
%======================================================
%======================================================
\section{Tutte le Matrici e non solo Frobenius}
%======================================================
%======================================================

\subsection{lemmetti di servizio}

\begin{lemma}\label{nil}
Sia $M=(m_{ij})$ una matrice $n\times n$ di polinomi di Laurent su $\Z_{p^k}$.
Supponiamo che per un certo $h<n$ sia $\modulo{M^h}{{p^k}}=0$.
Allora i coefficienti del polinomio caratteristico (modulo $\Z_{p^k}$) sono nulli.
\end{lemma}
\begin{proof}
$M$ � nilpotente e quindi il suo polinomio caratteristico � $y^n$.
\end{proof}



\begin{lemma}\label{lemmetto}
Siano $a, b, p, k$ numeri interi con $p$ primo e maggiore di $1$, $k>0$, $0\leq b < p^k$ e $\gcd(a,p)= 1$.
Allora $\modulo{ab}{p^k}=0$ implica $b=0$.
\end{lemma}
\begin{proof}
Supponiamo per assurdo che $\modulo{ab}{p^k}=0$ e $b>0$.
Visto che $\modulo{ab}{p^k}=0$ abbiamo che $p^k$ divide $ab$. 
Sia $a=a_1\cdot \cdots \cdot a_s$ e $b=b_1\cdot \cdots \cdot b_t$ la scomposizione in fattori primi di $a$ e $b$ rispettivamente.
Visto che $\gcd(a,p)= 1$ abbiamo che $a$ non divide $a$. Quindi $p^k$ deve dividere $b$, ma $b<p^k$ e quindi $p^k$ non divide nemmeno $b$. Ne segue la tesi.
\end{proof}

\begin{lemma}\label{fibodz}
Sia $p$ un numero primo maggiore di $1$. Sia $k$ un intero maggiore di $0$.
Sia $h$ un intero maggiore di zero.
Siano $n_1,\dots,n_h$ numeri interi maggiori di zero e tali che
$n_1<n_2<\cdots <n_h$.
Siano $\alpha_1,\dots,\alpha_h$ numeri interi compresi tra $1$ e $p^k-1$ 
tali per cui $\gcd(\alpha_i,p)=1$ ovvero $p$ non divide $\alpha_i$.
% $\modulo{\alpha_i}{p^h}\neq 0$.
Sia
\begin{eqnarray}\label{eq1}
T(n)&=&\modulo{\alpha_1 T(n-n_1)+\cdots + \alpha_h T(n-n_h)}{p^k}\\
T(n_h)&=&t_h\\
\cdots &=& \cdots\\
T(1)&=&t_1
\end{eqnarray}
con $t_i$ (valori iniziali della successione $T(n)$ non calcolabili ricorsivamente) compresi tra $0$ e $p^k -1$.
Supponiamo che esista almeno un indice $d$ con $1\leq d \leq n_h$ tale che $t_d\neq 0$.
Allora per infiniti valori di $n$ abbiamo
$$T(n) \neq 0$$
\end{lemma}

\begin{proof}
Chiamiamo $dz$ il numero dei $T(n)$ diversi da zero con $n\geq 0$. Supponiamo per assurdo $dz$ sia un numero finito maggiore di $0$. Allora esiste $h_0\geq 0$ tale che
$T(h_0) \neq 0$ e per ogni $n$ maggiore di $h_0$ abbiamo $T(n) = 0$.
Usando l'equazione (\ref{eq1})
calcoliamo $T(n)$ quando $n=n_h+h_0$ e otteniamo 
\begin{equation}\label{eq2}
T(n_h+h_0)=\modulo{\alpha_1T(n_h+h_0-n_1)+\cdots + \alpha_{h-1} T(n_h +h_0 - n_{h-1}) + \alpha_h T(h_0)}{p^k}
\end{equation}
Visto che per ipotesi per ogni $n>h_0$ abbiamo che $T(n) = 0$  dalla equazione (\ref{eq2})
abbiamo che 
\begin{equation}\label{eq3}
0=\modulo{\alpha_h T(h_0)}{p^k}
\end{equation}
Ma se $\modulo{\alpha_h T(h_0)}{p^k}=0$   significa che $p^k$ divide  $\alpha_h T(h_0)$. Dal Lemma \ref{lemmetto} possiamo concludere che per forza $T(h_0)= 0$ che contraddice l'ipotesi iniziale.
Concludiamo quindi che $dz$ � infinito oppure $dz=0$. Ma $dz$ non pu� essere uguale a $0$ perch� per ipotesi $T(d)\neq 0$ e quindi $dz$ deve valere almeno $1$. Quindi concludiamo che $dz$ deve essere infinito e quindi la tesi � dimostrata.
 \end{proof}

\subsection{traccia di ragionamento per la sensitivit� di matrici non frobenius}

Nota: ragioneremo nel seguito sulla sensitivit� da un lato (esponenti positivi), ma tutta la linea di ragionamento rimane vera 
anche con esponenti negativi e sensitivit� dall'altro lato.\\
Nota: per semplicit� e senza perdere di generalit� useremo una matrice $3\times 3$.\\

\noindent
Sia $M=(m_{ij})$ una matrice $3\times 3$ di polinomi di Laurent  con polinomio caratteristico
$ y^3-ay^2-by-c=0$. 

\noindent
Sappiamo che  
 $$\forall m\geq 3:\ \ \ M^m=a M^{m-1}+ b M^{m-2} + c M^{m-3}$$.
Quindi abbiamo
\begin{eqnarray*}
M^0 &=& I \ \ \ caso\ base \\
M^1 &=& M \ \ \ caso\ base\\
M^2 &=& M^2 \ \ \ caso\ base\\
M^3 &=& a M^2 +b M +c I \ \ da\ qui\ in\ avanti\ M^i si\ valuta\ ricorsivamente\\
M^4 &=& a M^3 +b M^2 +c M \\
&=&a (a M^2 +b M +c I) +b M^2 +c M\\
&=&(a^2+b) M^2 +(ab+c) M +ac I 
\end{eqnarray*}

\noindent
Prendiamo adesso un albero cos� definito (vedi Figura \ref{fig1}): \\
- radice: corrisponde a $M^m$\\
- ogni nodo ha tre figli che corrispondono a $M^{m-1},M^{m-2},M^{m-3}$\\
- gli archi sono etichettati con $a,b,c$.\\
- le foglie corrispondono a $M^2,M,I$

\noindent Nota: negli alberi ci sono i livelli (vedi ad esempio Figura \ref{fig1} che ha $7$ livelli, da $0$ a $6$). Un arco attraversa $k$ livelli quando 
nel lato destro della ricorsione moltiplica $M^{m-k}$.



\begin{figure}[htbp] 
        \centering
     \includegraphics[height=6cm]{./IMG_0449.jpg}
    \caption{Albero per calcolare $M^6$ }
    \label{fig1}
   \end{figure}
   
  Per ritrovare i risultati delle equazioni ricorsive basta fissare un nodo con l'altezza giusta e prendere tutti i cammini
  da quel nodo alle foglie, per ogni cammino si moltiplicano tra loro tutte le etichette degli archi che lo compongono e la matrice corrispondente della foglia  e poi si sommano tutte 
  le produttorie cosi ottenute. Si veda la Figura \ref{fig2} relativa al calcolo di $M^4$
  
  \begin{figure}[htbp]
        \centering
     \includegraphics[height=6cm]{./IMG_0450.jpg}
    \caption{Albero per calcolare $M^4$ }
    \label{fig2}
   \end{figure}

 Adesso consideriamo una matrice $M$ i cui elementi (che sono polinomi) non contengano monomi con coefficiente multiplo di $p$.
Inoltre trasformiamo $a,b,c$ come segue. Prima di tutto eliminiamo tutti i monomi di grado non massimo e poi eliminiamo del tutto i monomi che non hanno 
 "velocit�" massima  (la velocit� di un monomio associato ad un arco che collega il livello $h$ 
 al livello $k$ di un albero, si veda Figura \ref{fig3}, � data dall'esponente del monomio diviso $h-k$, in altre parole � l'esponente del monomio che etichetta un arco diviso il numero di livelli che l'arco attraversa).\\
 Esempio: siano $a=x^{-3}+3x+x^2, b=2 x^2 + x^3,c=3x^2+2x^6$ su $\Z_{49}$.
 prima calcoliamo $a'=x^2, b'=x^3,c'=2x^6$ e poi visto che $a'$ ha velocit� $2/1=2$,
 $b'$ ha velocit� $3/2$ e $c'$ ha velocit� $6/3=2$, abbiamo $a''=x^2, b''=0,c''=2x^6$.
 
 La velocit� di espansione di un albero � proprio l'incremento di esponente che abbiamo su un qualsiasi cammino
 scendendo di un livello nell'albero si veda la Figura \ref{fig3} per capire meglio
  \begin{figure}[htbp]
        \centering
     \includegraphics[height=6cm]{./IMG_0451.jpg}
    \caption{esempio di velocit� di aumento dell'esponente }
    \label{fig3}
   \end{figure}
 
  
 \begin{teo}\label{stesso grado}
 Sosteniamo che (da dimostrare) presi due cammini nell'albero (con i nuovi pesi $a'',b'',c''$ sugli archi) 
 che vanno dalla radice ad uno stesso livello $k$ dell'albero
 e calcolati i valori (prodotti delle etichette) relativi ai due cammini otteniamo due monomi con lo stesso grado
  \end{teo}
  
  \begin{teo}\label{stesso vel}
 Sosteniamo che (da dimostrare) i due alberi con pesi $a,b,c$ e  con  pesi $a'',b'',c''$  hanno la medesima velocit� di espansione
   \end{teo}
  
  Dividiamo adesso  l'albero in due zone, la zona base con i livelli che vanno da $0$ a $n-1$ e la zona ricorsione con i livelli che vanno da $n$ a $m$.
  Inoltre adesso concentriamoci su una certa entry della matrice invece che su tutta la matrice (che poi sar� la entry che vogliamo dimostrare che diverge in grado quando $m$ tende all'infinito), ad esempio la entry in angolo (posizione $(n,n)$).
  
  Tutti i cammini  partono dalla radice (livello $m$) e  terminano in uno dei livelli della zona base dove "acquistano qualche grado in pi�" dovuto alla moltiplicazione con una potenza "base" della matrice (o di un singolo elemento delle potenze di base della matrice, se stiamo ragionando di singoli elementi).
Tutti i cammini che arrivano a un certo livello di base $k$ hanno lo stesso esponente per il teorema \ref{stesso grado}.
L'esponente si pu� calcolare ed � uguale alla velocit� di espansione $v$ (che ricordiamo � quanto aumenta l'esponente ad ogni livello) moltiplicata per $m-k$ dove $k$ � il livello base dove il cammino termina ($m-k$ � il numero di livelli attraversati dal cammino).
A questa quantit� va aggiunto l'incremento di esponente dovuto alla moltiplicazione per un elemento di una potenza della matrice (elemento di base). Supponiamo che per il livello $k$ abbiamo un incremento di $\Delta_k$. 
Quindi i cammini col massimo esponente avranno esponente 
$$\max_{0\leq k \leq n-1} \{v (m-k)+\Delta_k\}$$ 
Supponiamo che il massimo si raggiunga per $k=k'$ (o anche a parimerito per pi� valori di $k$) .
Abbiamo a questo punto che 
l'esponente massimo raggiungibile da un cammino sar� 
$$espmax=v (m-k')+\Delta_{k'}$$
Dove $v (m-k')$ � l'esponente accumulato sul cammino prima del caso base e $\Delta_{k'}$ � l'incremento di esponente dovuto al caso base.
Ma siccome tutti i conti si fanno modulo $p^k$ occorre che il coefficiente $C$ di $x^{espmax}$ sia 
diverso da $0$ modulo $p^k$
Ma come lo calcoliamo $C$ ?

Lo calcoliamo con la seguente  equazione ricorsiva dove $a''',b''',c'''$ sono ottenuti da $a'',b'',c''$ dove al posto di $x$ mettiamo $1$ (cos� facendo i monomi diventano i coefficienti dei monomi).

 $$\forall m\geq 3:\ \ \ C (m)=a''' C(m-1)+ b''' C(m-2) + c''' C(m-3)$$
 Per quanto riguarda i casi base della ricorsione, bisogna prendere il monomio di grado massimo degli elementi 
 (se si ragiona sugli elementi singoli)
 delle potenze di base della matrice, ma solo quelli  che hanno velocit� massima (quelli che determinano il $k'$ di cui si parlava un po' sopra), 
 gli altri si mettono a $0$.
 
 
 \begin{teo}\label{divergence}
 Sosteniamo che $C(m)$ � diverso da zero per infiniti valori di $m$. Da qui la sensitivit� dell'automa originario
   \end{teo}

}
\end{comment}


==> old.tex <==
%======================================================
\section{Characteristic Polynomial}
%======================================================
%======================================================

Sia $M(x)$ la matrice associata a $F$. 
Siano $\lambda_i$ gli autovalori di $M(x)$. In generale $\lambda_i$  possono dipendere da $x$ e possono non essere polinomi di Laurent.
Prendiamo $M(x)$ di dimensione $3$. Il polinomio caratteristico di $M(x)$ pu\`o essere scritto come segue
$$P_M(y)= y^3 - y^2 (\lambda_1 +\lambda_2+\lambda_3)+y (\lambda_1 \lambda_2+\lambda_1\lambda_3+\lambda_2\lambda_3)-
\lambda_1\lambda_2\lambda_3
$$
inoltre
$$P_{M^n}(y)= y^3 - y^2 (\lambda_1^n +\lambda_2^n+\lambda_3^n)+y ((\lambda_1 \lambda_2)^n+(\lambda_1 \lambda_3)^n+(\lambda_2 \lambda_3)^n)-
(\lambda_1\lambda_2\lambda_3)^n$$
con $\lambda_1^n +\lambda_2^n+\lambda_3^n$, $(\lambda_1 \lambda_2)^n+(\lambda_1 \lambda_3)^n+(\lambda_2 \lambda_3)^n$ e 
$(\lambda_1\lambda_2\lambda_3)^n$ polinomi in $x$ e $x^{-1}$.
\noindent
In generale i coefficienti di $P_{M^n}(y)$ possono essere scritti in funzione degli autovalori nel modo seguente.
Il coefficiente di $y^i$ \`e  la sommatoria  di tutti i prodotti dei sottoinsiemi di esattamente $dimensione\ della\ matrice - i$ autovalori. Il segno \`e da definire ma per i nostri ragionamenti \`e trascurabile.

%======================================================
%======================================================
\section{Propriet\`a coefficienti del polinomio caratteristico}
%======================================================
%======================================================
In questa sezione dimostriamo che se esiste un coefficiente sensitivo
del polinomio caratteristico di una matrice $M$ che definisce un MCA  allora
le potenze di $M$ hanno  infiniti polinomi caratteristici distinti. Ci\`o implica che le potenze di $M$ sono infinite. 
Ci\`o implica che l'automa \`e sensitivo.

\begin{teo}\label{symmetric}
Sia $R$ un anello commutativo. Sia $p(x_1,\dots,x_n)$ un polinomio simmetrico nelle variabili $x_1,\dots,x_n$ 
a coefficienti in $R$.
Allora $$p(x_1,\dots,x_n)=q(e_1(x_1,\dots,x_n),\dots,e_n(x_1,\dots,x_n))$$ 
dove $q(y_1,\dots, y_n)$ \`e un polinomio a coefficienti in $R$ e $e_i(x_1,\dots,x_n)$ sono i polinomi simmetrici elementari
in $x_1,\dots,x_n$.
\end{teo}


\begin{lemma}\label{cpc0}
Sia $p$ primo maggiore di $1$ e $h$ intero maggiore di zero. Siano $k_1,\dots , k_l$ 
numeri interi positivi tali per cui $k_1+\cdots + k_l = p^h$.
Allora il coefficiente multinomiale ${{p^h}\choose{k_1,\dots,k_l}} = \frac{p^h !}{k_1! \cdot \cdots \cdot k_l!}$
\`e sempre multiplo di $p$ tranne nel caso in cui $l=1$ e $k_1=p^h$.

\end{lemma}



\begin{lemma}\label{cpc1}
Sia $p$ primo maggiore di $1$. Sia $k$ intero maggiore di $1$.
Sia $c(x)$  un polinomio  di Laurent con coefficienti presi in $\Z_{p^k}$ non divisibili per $p$.
Sia $c(x)= a_1+\cdots +a_s$ una riscrittura di $c(x)$ arbitraria con $a_i$ non necessariamente polinomi tale per cui
$\modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}$ sia un polinomio di Laurent con coefficienti  in $\Z_{p^k}$.
\noindent
Allora per ogni $h$ intero maggiore o uguale a $0$ 
esiste un polinomio $\alpha$ di Laurent con coefficienti  in $\Z_{p^k}$
tale per cui 

$$ \modulo{(a_1+\cdots +a_s)^{p^h}}{p^k}= \modulo{a_1^{p^h}+\cdots +a_s^{p^h}+
p \alpha}{p^k}$$

\end{lemma}
\begin{proof}
Basta usare la formula dello sviluppo multinomiale e applicare il Lemma \ref{cpc0}.

\end{proof}


\begin{lemma}\label{cpc2}
Sia $p$ primo maggiore di $1$. Sia $k$ intero maggiore di $1$.
Sia $c(x)$  un polinomio  di Laurent con coefficienti presi in $\Z_{p^k}$ non divisibili per $p$.
Assumiamo che $c(x)$ sia sensitivo  ovvero che $d^+ >0$ oppure $d^->0$. Senza perdere di generalit\`a
assumiamo $d^+ >0$.
Sia $c(x)= a_1+\cdots +a_s$. Assumiamo inoltre che  per ogni $h\geq 0$  
$\modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}$ sia un polinomio di Laurent con coefficienti  in $\Z_{p^k}$.
\noindent
Allora per ogni $h$ intero maggiore o uguale a $0$ vale
$$deg\left[\modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}\right] \geq deg\left[\modulo{(a_1+\cdots +a_s)^{p^h}}{p^k}\right]=  d^+ p^h$$

\end{lemma}
\begin{proof}
Riscriviamo  $c(x)$ come $c(x)=q(x)+ a x^{d^+}$ dove $a x^{d^+}$ \`e il monomio di grado massimo in $c(x)$ e quindi 
 $deg[q(x)]< d^+$ e $\gcd(a,p)=1$. 
Usando un po' di algebra elementare possiamo concludere che 
$\modulo{c(x)^{p^h}}{p^k}=\modulo{(q(x)+ a x^{d^+})^{p^h}}{p^k}= 
\modulo{q'(x)+ a^{p^h}x^{p^hd^+}}{p^k}$ con $deg[q'(x)]<p^hd^+$.
Ma $\modulo{q'(x)+ a^{p^h}x^{p^hd^+}}{p^k}= q''(x)+a'x^{p^hd^+} $ con $a'=\modulo{a^{p^h}}{p^k}$ e quindi
$a'$ diverso da zero e non divisibile per $p$. Questo dimostra che 
$deg\left[\modulo{(a_1+\cdots +a_s)^{p^h}}{p^k}\right]=  d^+ p^h$.\\
\noindent
Dal Lemma \ref{cpc1} sappiamo che 
$$ \modulo{(a_1+\cdots +a_s)^{p^h}}{p^k}= \modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}+
p \alpha$$ 
e dal teorema \ref{symmetric} possiamo dedurre che  $\alpha$ 
\`e un polinomio 


e quindi concludiamo che il polinomio $ \modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}+
p \alpha$ deve contenere il monomio $a'x^{p^hd^+}$.
Se $p \alpha$ (che per ipotesi \`e un polinomio) non contenesse il monomio di grado $p^hd^+$ allora 
avremmo dimostrato che  $a'x^{p^hd^+}$ deve essre contenuto in $\modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}$ e quindi
$deg\left[\modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}\right] \geq p^hd^+ = deg\left[\modulo{(a_1+\cdots +a_s)^{p^h}}{p^k}\right]$.
% in quanto sarebbe $\modulo{a_1^{p^h}+\cdots +a_s^{p^h}}{p^k}$ a doverlo contenere.
Se viceversa $p \alpha$   contenesse il monomio di grado $p^hd^+$ allora Sarebbe della forma $p a'' x^{p^hd^+}$
e quindi dentro a $\modulo{(a_1+\cdots +a_s)^{p^h}}{p^k}$ dovrebbe starci un monomio $a''' x^{p^hd^+}$
tale che $a''' x^{p^hd^+} + p a'' x^{p^hd^+} = a' x^{p^hd^+}$.
Dovrebbe quindi valere che $a'''+pa''=a'$. Visto che $a'$ non \`e divisibile per $p$ questo significa che anche $a'''$ non pu\`o essere divisibile per $p$ e questo dimostra la tesi.
\end{proof}



\begin{teo}\label{cpc3}
Sia $M(x)$ la matrice associata a un MCA $F$ su $\Z_{p^k}$.
Sia 
$$p^{(i)}(y)= y^n + c^{(i)}_n(x) y^{n-1}+ \cdots + c^{(i)}_1(x) y^{1}+c^{(i)}_0(x) $$
il polinomio caratteristico di $M^i(x)$.
Se  $c^{(1)}_j(x)$ un qualsiasi coefficiente di $p^{(1)}(y)$. Sia $d^+ =deg[c^{(1)}_j(x)] >0$.
Assumiamo che nessun coefficiente di $c^{(1)}_j(x)$ sia divisibile per $p$.
Allora $deg[c^{(i)}_j(x)]$ \`e illimitato ovvero $$\limsup_{i \to \infty} deg[c^{(i)}_j(x)] = \infty$$
\end{teo}
$c^{(1)}_j(x)$ \`e un coefficiente del polinomio caratteristico di $M$. Ogni coefficiente di ogni polinomio caratteristico
si pu\`o scrivere come la sommatoria di produttorie degli autovalori. Se si eleva alla potenza $i$
la matrice, il coefficiente del polinomio caratteristico diventa la sommatoria delle stesse produttorie elevate (ognuna) alla potenza $i$. Possiamo quindi applicare il Lemma \ref{cpc2} e la tesi \`e dimostrata.

%======================================================


==> smca-gen.tex <==
%======================================================
%======================================================
\section{Sensitivity per MCA generali}
%======================================================
%======================================================

Sia $F$ un $MCA$ definito da 
$$M(x) = \modulo{\sum_{i=-r}^{r} M_i x^{-i}}{m}$$.


\begin{teo}\label{uno}
Let $F$ an MCA defined by the matrixes 
$\M_{-r},\dots,\M_0,\dots,\M_r\in \mat{n}{\z_m}$.
The following statements are equivalent:
\begin{enumerate}
\item $F$ is sensitive to the initial conditions;
\item
$\limsup_{t\to\infty} deg[M(X)^t]= \infty$;
\item
$|\{ M(X)^i,\ i\geq 1 \}|=\infty$;
\item $F$ is not equicontinuous (la condizione del teo VECCHIO mi pare equivalente alla negazione di 2)
\end{enumerate}

\end{teo}

VECCHIO:
\begin{teo}\label{due}
$F$  \`e equicontinuo (nei lineari: non sensitivo) se e solo se esiste un  intero positivo $k$ tale che:
$$\max_{n \geq 1} deg[M^n(x)] \leq k$$.
\end{teo}



\begin{ex}
$$M(x)=
\begin{bmatrix}
0& 1 \\
0 & 0
\end{bmatrix}
+
\begin{bmatrix}
0& 0 \\
1 & 0
\end{bmatrix}
x = 
\begin{bmatrix}
0& 1 \\
x & 0
\end{bmatrix}
$$
Autovalori = $(-\sqrt(x),\sqrt(x))$.
L'automa \`e sensitivo essendo la radice dello shift ovvero $F^2(x)=\sigma(x)$. Si noti che $M^2(x)=
\begin{bmatrix}
x& 0 \\
0 & x
\end{bmatrix}
$.
\end{ex}




%======================================================

